Average Sensitivity of Dynamic Programming

When processing data with uncertainty, it is desirable that the output of the algorithm is stable against small perturbations in the input. Varma and Yoshida [SODA'21] recently formalized this idea and proposed the notion of average sensitivity of algorithms, which is roughly speaking, the average Hamming distance between solutions for the original input and that obtained by deleting one element from the input, where the average is taken over the deleted element. In this work, we consider average sensitivity of algorithms for problems that can be solved by dynamic programming. We first present a $(1-\delta)$-approximation algorithm for finding a maximum weight chain (MWC) in a transitive directed acyclic graph with average sensitivity $O(\delta^{-1}\log^3 n)$, where $n$ is the number of vertices in the graph. We then show algorithms with small average sensitivity for various dynamic programming problems by reducing them to the MWC problem while preserving average sensitivity, including the longest increasing subsequence problem, the interval scheduling problem, the longest common subsequence problem, the longest palindromic subsequence problem, the knapsack problem with integral weight, and the RNA folding problem. For the RNA folding problem, our reduction is highly nontrivial because a naive reduction generates an exponentially large graph, which only provides a trivial average sensitivity bound.

==> old/2d.tex <==
\section{Two-dimensional DP}

Let $V=[0, n]\times [0, m]$ be a two-dimensional grid. Let $E$ be a set of edges on $V$. Each edge is a form of $(x,y) \to (x',y')$ with $x\leq x'$, $y\leq y'$ and $(x,y)\neq (x',y')$. Each edge $e$ has a weight $w(e)$.


\begin{algorithm}[t!]
\caption{Less-sensitive Maximum Weight Chain $f(U)$}
\begin{algorithmic}[1]\label{alg:main}
\STATE Sample $t$ from the uniform distribution over $[1,n+m]$
\STATE Sample $c$ from the uniform distribution over $\left[\frac{\epsilon \OPT(U)}{\log(|U|\epsilon^{-1})},2\cdot \frac{\epsilon \OPT(U)}{\log(|U|\epsilon^{-1})} \right]$
\IF{$t\leq n$}
    \STATE Let $E_t=\{e=((i,j),(i',j')): e\in E, i<t\leq i'\}$
\ELSE
    \STATE Let $E_t=\{e=((i,j),(i',j')): e\in E, j<t-n\leq j'\}$
\ENDIF
\FOR{$e\in E_t$}
    \STATE Let $r(e)$ be the maximum value that uses $e$
\ENDFOR
\STATE Sample $\bar{e}\in E_t$ with probability proportional to $\exp(r(\bar{e})/c)$
\RETURN $f(G_{-e})\cup \{\bar{e}\}\cup f(G_{+e})$
\end{algorithmic}
\end{algorithm}

For the purpose of analysis, we consider that each ...


First we analyze the approximation factor. First we analyze the loss by the exponential mechanism.

\begin{lemma}
We have 
\begin{align}
    \E[r(\bar{e})]\geq (1-2\epsilon) \OPT(G).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    \Pr[r(\bar{e}) \leq (1-\epsilon)\OPT(G)]
    &= \frac{\sum_{e\in E_t, r(e)\leq (1-\epsilon) \OPT(G)}\exp(r(e)/c)}{\sum_{v\in E_t}\exp(r(e)/c)}\\
    &\leq \frac{|E_t|\exp((1-\epsilon)\OPT(G)/c)}{\sum_{v\in E_t}\exp(r(e)/c)}\\
    &\leq \frac{|E_t|\exp((1-\epsilon)\OPT(G)/c)}{\exp(\OPT(G)/c)}\\
    &= |E_t|\exp(-\epsilon \cdot \OPT(G)/c)\\
    &= |E_t|\cdot \frac{\epsilon}{|E|}\\
    &\leq \epsilon.
\end{align}

Therefore, we have
\begin{align}
    \E[r(\bar{e})]
    &\geq (1-\epsilon)(1-\epsilon)\OPT(U)\\
    &\geq (1-2\epsilon)\OPT(U).
\end{align}
\end{proof}


Next, we analyze the loss by the recursion.

\begin{lemma}
We have
\begin{align}
    \E\left[w(f(G))\right]\geq (1-7\epsilon\log (n+m))\OPT(G).
\end{align}
\end{lemma}
\begin{proof}
We prove by induction on $n+m$. If $n+m=0$, the statement is clear.
Now, we have
\begin{align}
    \E\left[w(f(G))\right]
    &= \frac{1}{n+m}\E\left[\sum_{t=1}^{n+m}\sum_{e\in E_t}\Pr[e=\bar{e}]\left(\E\left[w(f(G_{-e}))\right]+w(e)+\E\left[w(f(G_{+e}))\right]\right)\right]\\
    &= \frac{1}{n+m}\E\left[\sum_{t=1}^{n}\sum_{e\in E_t}\Pr[e=\bar{e}]\left((1-7\epsilon \log (t-1+m)\OPT(G_{-e})+w(e)+(1-7\epsilon \log (n+m-t))\OPT(G_{-e})\right)\right]\\
    &+ \frac{1}{n+m}\E\left[\sum_{t=n+1}^{n+m}\sum_{e\in E_t}\Pr[e=\bar{e}]\left((1-7\epsilon \log (t-1))\OPT(G_{-e})+w(e)+(1-7\epsilon \log (2n+m-t))\OPT(G_{-e})\right)\right]\\
    &= \frac{1}{n+m}\E\left[\sum_{t=1}^{n+m}\sum_{e\in E_t}\Pr[e=\bar{e}]\left((1-7\epsilon \log (i+j))\OPT(G_{-e})+w(e)+(1-7\epsilon \log (n+m-i'-j'))\OPT(G_{-e})\right)\right]\\
    &\geq \E\left[\sum_{e\in E_t}\Pr[e=\bar{e}]\left((1-7\epsilon \log (n+m))\OPT(G_{-e})+(1-7\epsilon \log |U_{+v}|)\OPT(U_{+v})\right)\right]+1\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left(\OPT(U_{-v})+\OPT(U_{+v})\right)\right]+1\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]r(v)\right]\\
    &= \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[r(\bar{v})\right]\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right)(1-2\epsilon)\OPT(U)\\
    &\geq \left(1-7\epsilon\log \left(\frac{3}{4}\OPT(U)\right)-2\epsilon \right)\OPT(U)\\
    &\geq (1-7\epsilon\log \OPT(U))\OPT(U).
\end{align}
\end{proof}


Next we analyze the sensitivity. Since the algorithm is symmetric over axes, without loss of generality we can assume that the element of the first axis is removed.
To evaluate the earth mover's distance, we recursively transport the probability. We transport the probability so that the choice of cutting direction (vertical or horizontal), cutting place, and choice of $\bar{e}$. First, we analyze the loss by choosing 

\begin{lemma}

\end{lemma}

==> old/RNA_broken.tex <==

\subsection{RNA Folding}
The \emph{RNA folding problem} is defined as follows.
\begin{prb}[RNA folding Problem]
Let $A$ be a string of length $n$ over the alphabet $\Sigma$. Let $\mathcal{R}\subseteq \Sigma\times \Sigma$ be a binary relation. Two pairs of indices $(l,r)$ and $(l',r')$ are \emph{pseudoknot} if exactly one of $l'$ and $r'$ is located between $l$ and $r$. The output is a set of pairs of indices $\{(l_1,r_1),\dots,(l_t,r_t)\}$ such that any two of $l_1,r_1,\dots, l_t,r_t$ are distinct. Maximize $t$, subject to $l_i < r_i$ and $(A_{l_i},A_{r_i})\subseteq \mathcal{R}$ for all $i\in \{1,\dots, t\}$ and no two different pair forms a pseudoknot.
\end{prb}
The distance between two solution $X_1,X_2$ is defined by $|X_1\triangle X_2|$, where we see $X_i$ as a set of pairs.
The algorithm first samples a parameter $L$ from uniform distribution over $[\log n, 2\log n]$.

Let us construct a graph $G$ to apply Algorithm~\ref{alg:main}. 
The integer quadraple $(l,p,q,r)$ is \emph{well-ordered} if $l\leq p<q\leq r$.
Each vertex of $G$ is represented by a list of the well-ordered quadraples of indices $((l_1,p_1,q_1,r_1),\dots,(l_k,p_k,q_k,r_k))$ of length at most $L$ that satisfies all the following conditions.
\begin{enumerate}
    \item[(i)] $0\leq l_j<r_j\leq n+1$ and $1\leq p_j<q_j\leq n$ for all $j$.
    \item[(ii)] $(A_{p_j},A_{q_j})\in \mathcal{R}$ holds for all $j$.
    \item[(iii)] $(l_k,r_k)=(p_k,q_k)$.
    \item[(iv)] $l_j<l_{j'}<r_{j'}<r_j$ and $[p_j,q_j]\cap [l_{j'},r_{j'}]=\emptyset$ hold for all $j < j'$.
\end{enumerate}
For each vertex $v\in V(G)$, the weight of $v$ is $1$.

For two well-ordered quadraples $(l,p,q,r)$ and $(l',p',q',r')$, we define a partial order $\preceq$ by $(l,p,q,r)=(l',p',q',r')$, $r<l'$ or $p\leq l'<r'\leq q$. We prepare an edge from the vertex $((l_1,p_1,q_1,r_1),\dots,(l_k,p_k,q_k,r_k))$ to $((l'_1,p'_1,q'_1,r'_1),\dots,(l'_{k'},p'_{k'},q'_{k'},r'_{k'}))$ if the former is lexicographically strictly smaller than the latter, where we compare each quadraples by the order $\preceq$. The next lemma ensures that $\preceq$ is indeed a partial order. That also ensures that $G$ is acyclic and transitive.
\begin{lemma}
$\preceq$ is a partial order.
\end{lemma}
\begin{proof}
The reflexivity of $\preceq$ is clear from the definition. 
Now, we prove $\prec$ is asymmetric. 
Assume $(l,p,q,r)\neq (l',p',q',r')$ satisfies $(l,p,q,r)\prec (l',p',q',r')\prec (l,p,q,r)$. 
If $r<l'$ and $r'<l$, we have $l<r<l'<r'<l$ and it is contradiction. 
If $r<l'$ and $p'\leq l<r\leq q'$, we have $r<l'\leq p'<r$ and it is contradiction. 
The same argument holds for the case $p\leq l'<r'\leq q$ and $r<l'$. 
If $p\leq l'<r'\leq q$ and $p'\leq l<r\leq q'$, we have $l \leq p \leq l'\leq p'\leq l$ and $r\leq q'\leq r'\leq q\leq r$ and therefore we have $(l,p,q,r)=(l',p',q',r')$.
Therefore $\prec$ is asymmetric.

Finally, we prove $\prec$ is transitive. 
Assume $(l,p,q,r)\neq (l',p',q',r')\neq (l'',p'',q'',r'')$ satisfies $(l,p,q,r)\prec(l',p',q',r')\prec(l'',p'',q'',r'')$. 
We prove that $(l,p,q,r)\prec (l'',p'',q'',r'')$. 
If $r<l'$ and $r'<l''$, we have $r<l'<r'<l''$. Therefore we have $r<l''$ and the statement holds. 
If $r<l'$ and $p'\leq l''<r''\leq q'$, we have $r<l'\leq p'\leq l''$. Therefore we have $r<l''$ and the statement holds. 
The same argument holds for the case $p\leq l'<r'\leq q$ and $r'<l''$???\snote{kowareteru}. 
If $p\leq l'<r'\leq q$ and $p'\leq l''<r''\leq q'$, we have $p\leq l' \leq p'\leq l'' < r''\leq q' \leq r'\leq q$. Therefore we have $p\leq l''<r''\leq q$ and the statement holds.
Therefore $\prec$ is transitive and thus a partial order.
\end{proof}

Let us make a correspondence between a path of $G$ and a solution of the original problem. Let $P=(v_1,\dots, v_t)$ be a path of $G$. Let $v_i=((l_{i,1},p_{i,1},q_{i,1},r_{i,1}),\dots,(l_{i,k_i},p_{i,k_i},q_{i,k_i},r_{i,k_i}))$. The solution is obtained by matching $l_{i,k_i}$ and $r_{i,k_i}$ for all $i$. We prove that the solution obtained in this way does not contain a pseudoknot.
\begin{lemma}
For $i < i'$, we have either $l_{i,k_i}<l_{i',k_{i'}}<r_{i',k_{i'}}<r_{i,k_i}$ or $[l_{i,k_i},r_{i,k_i}]\cap [l_{i',k_{i'}},r_{i',k_{i'}}]=\emptyset$.
\end{lemma}
\begin{proof}
If $v_i$ is a prefix of $v_{i'}$, we have 
\begin{align}
    [l_{i,k_i},r_{i,k_i}]\cap [l_{i',k_{i'}},r_{i',k_{i'}}]
    &= [p_{i,k_i},q_{i,k_i}]\cap [l_{i',k_{i'}},r_{i',k_{i'}}]\\
    &= [p_{{i'},k_i},q_{{i'},k_i}]\cap [l_{i',k_{i'}},r_{i',k_{i'}}]=\emptyset,
\end{align}
where the first equality is from the condition (iii), the second equality is from the fact that $v_i$ is a prefix of $v_{i'}$, and the last equality is from $k_i<k_{i'}$ and the condition (iv).

Assume $v_i$ is not a prefix of $v_{i'}$ and let $j$ be the first index that $(l_{i,j},p_{i,j},q_{i,j},r_{i,j})\neq (l_{i',j},p_{i',j},q_{i',j},r_{i',j})$. From the definition of $\prec$, $r_{i,j}<l_{i',j}$ or $p_{i,j}\leq l_{i',j}<r_{i',j}\leq q_{i,j}$ holds. If $r_{i,j}<l_{i',j}$, we have
\begin{align}
    [l_{i,k_i},r_{i,k_i}]\cap [l_{i',k_{i'}},r_{i',k_{i'}}]
    &\subseteq [l_{i,j},r_{i,j}]\cap [l_{i',j},r_{i',j}]=\emptyset,
\end{align}
where the set inequality is from the condition (iv) and the equality is from $r_{i,j}<l_{i',j}$. If $p_{i,j}\leq l_{i',j}<r_{i',j}\leq q_{i,j}$ and $j=k_i$, we have
\begin{align}
    l_{i,k_i}=p_{i,k_i}=p_{i,j}\leq l_{i',j} \leq l_{i',k_{i'}} < r_{i',k_{i'}} \leq r_{i',j}\leq q_{i,j}=q_{i,k_i}=r_{i,k_i},
\end{align}
where the first and last equalities are from the condition (iii), the second and third equalities are from $j=k_i$, and the second and fourth inequalities are from $j\leq k_{i'}$ and the condition (iv).
If $p_{i,j}\leq l_{i',j}<r_{i',j}\leq q_{i,j}$ and $j < k_i$, we have
\begin{align}
    [l_{i,k_i},r_{i,k_i}]\cap [l_{i',k_{i'}},r_{i',k_{i'}}]
    &\subseteq [l_{i,j+1},r_{i,j+1}]\cap [l_{i',j},r_{i',j}]\\
    &\subseteq [l_{i,j+1},r_{i,j+1}]\cap [p_{i,j},q_{i,j}]=\emptyset,
\end{align}
where the first set inequality is from $j+1\leq k_i$, $j\leq k_{i'}$ and the condition (iv), the second set inequality is from $p_{i,j}\leq l_{i',j}<r_{i',j}\leq q_{i,j}$ and the last equality is from the condition (iv). Therefore, the lemma is proved.
\end{proof}

Now we consider the reverse direction of the correspondence. Let $\{(l_1,r_1),\dots, (l_t,r_t)\}$ be a feasible solution of the original problem. Let $T$ be a forest such that the vertex set is $\{(l_1,r_1),\dots, (l_t,r_t)\}\cup \{(0,n+1)\}$ and $(l,r)$ is an ancestor of $(l',r')$ if and only if $[l',r']\subseteq [l,r]$. Let us fix a heavy-light decomposition of $T$. The path of $G$ is obtained by the Algorithm~\ref{alg:makepath}.

\begin{algorithm}[t!]
\caption{Making a path}\label{alg:makepath}
\Procedure{\emph{\Call{Rec}{$l,r$}}}{
    \If{$(l,r)$ has no child}{
        \Return\;
    }
    Let $(l_h,r_h)$ be the heavy child of $(l,r)$\;
    Add $(l,l_h,r_h,r)$ to the last of $CurrentList$\;
    \For{light children $(l',r')$ of $(l,r)$ in increasing order of $l'$}{
        Add $(l',l',r',r')$ to the last of $Path$\;
        Add $CurrentList+(l',l',r',r')$ to the last of $Path$\;
        Remove $(l',l',r',r')$ from the last of $CurrentList$\;
        \Call{Rec}{$l',r'$}\;
    }
    Remove $(l,l_h,r_h,r)$ from the last of $CurrentList$\;
    Add $CurrentList+(l_h,l_h,r_h,r_h)$ to the last of $Path$\;
    \Call{Rec}{$l_h,r_h$}\;
}
\Procedure{\emph{\Call{MakePath}{}}}{
    Let $CurrentList$ and $Path$ be an empty list\;
    \Call{Rec}{$0,n+1$}\;
    \Return $Path$\;
}
\end{algorithm}



==> old/edgeweight.tex <==
\section{Edge Weight}

Let $G=(V,E)$ be a transitive directed acyclic graph. %For a vertex $v\in V$, let $(-\infty, v)$ be the set of vertices from which there is an edge to $v$, and $(v,\infty)$ be the set of vertices to which there is an edge from $v$. For two vertices $u,v\in V$, let $(u,v)=(u,\infty)\cap (-\infty,v)$. For simplicity, we write $V=(-\infty, \infty)$.
Assume a global ordering.


\begin{algorithm}[t!]
\caption{Less-sensitive Maximum Weight Chain $f(U)$}
\begin{algorithmic}[1]\label{alg:main}
\STATE Sample $c$ from the uniform distribution over $\left[\frac{\epsilon \OPT(U)}{\log(|U|^4\epsilon^{-1})},2\cdot \frac{\epsilon \OPT(U)}{\log(|U|^4\epsilon^{-1})} \right]$
\STATE Sample $t$ from the uniform distribution over $\left[1,n-1\right]$
\IF{$U=\emptyset$}
    \RETURN $\emptyset$
\ENDIF
\STATE Let $E_t$ be the set of edges from $\leq t$ to $>t$
\FOR{$e\in E$}
    \STATE Let $r(e)$ be the maximum weight of a chain that contains $e$
\ENDFOR
\STATE Sample $\bar{e}\in E_t$ with probability proportional to $\exp(r(\bar{e})/c)$
\RETURN $f(U_{-\bar{e}})\cup \{\bar{e}\}\cup f(U_{+\bar{e}})$
\end{algorithmic}
\end{algorithm}

The answer is $f(V)$.



First we analyze the approximation factor. First we analyze the loss by the exponential mechanism.

\begin{lemma}
We have 
\begin{align}
    \E[r(\bar{e})]\geq (1-2\epsilon) \OPT(U).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    \Pr[r(\bar{e}) \leq (1-\epsilon)\OPT(U)]
    &= \frac{\sum_{e\in E_t, r(e)\leq (1-\epsilon) \OPT(U)}\exp(r(e)/c)}{\sum_{e\in E_t}\exp(r(e)/c)}\\
    &\leq \frac{|E_t|\exp((1-\epsilon)\OPT(U)/c)}{\sum_{e\in E_t}\exp(r(e)/c)}\\
    &\leq \frac{|E_t|\exp((1-\epsilon)\OPT(U)/c)}{\exp(\OPT(U)/c)}\\
    &= |E_t|\exp(-\epsilon \cdot \OPT(U)/c)\\
    &= |E_t|\cdot \frac{\epsilon}{|U|^4}\\
    &\leq \epsilon.
\end{align}

Therefore, we have
\begin{align}
    \E[r(\bar{v})]
    &\geq (1-\epsilon)(1-\epsilon)\OPT(U)\\
    &\geq (1-2\epsilon)\OPT(U).
\end{align}
\end{proof}


Next, we analyze the loss by the recursion.

\begin{lemma}
We have
\begin{align}
    \E\left[w(f(U))\right]\geq (1-7\epsilon\log |U|)\OPT(U).
\end{align}
\end{lemma}
\begin{proof}
We prove by induction on $|U|$. If $|U|=1$, the statement is clear.
Now, we have
\begin{align}
    \E\left[w(f(U))\right]
    &= \E\left[\frac{1}{n-1}\sum_{t=1}^{n-1}\sum_{e\in E_t}\Pr[e=\bar{e}]\left(\E\left[w(f(U_{-e}))\right]+w(e)+\E\left[w(f(U_{+e}))\right]\right)\right]\\
    &\geq \E\left[\sum_{e\in E_t}\Pr[e=\bar{e}]\left((1-7\epsilon \log |U_{-e}|)\OPT(U_{-v})+(1-7\epsilon \log |U_{+v}|)\OPT(U_{+v})\right)\right]+1\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left(\OPT(U_{-v})+\OPT(U_{+v})\right)\right]+1\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]r(v)\right]\\
    &= \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[r(\bar{v})\right]\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right)(1-2\epsilon)\OPT(U)\\
    &\geq \left(1-7\epsilon\log \left(\frac{3}{4}\OPT(U)\right)-2\epsilon \right)\OPT(U)\\
    &\geq (1-7\epsilon\log \OPT(U))\OPT(U).
\end{align}
\end{proof}


Next we analyze the sensitivity. We denote $r(v)$ in the Algorithm~\ref{alg:main} on the instance $U\setminus \{u\}$ by $r^u(v)$.

To evaluate the earth mover's distance, we recursively transport the probability. We transport the probability so that the case of same choices of $c$, $d$, and $\bar{v}$ correspond to each other. For these cases, We recursively transport the probability from $\mathcal{A}(f(U_{-v}))$ to $\mathcal{A}(f(U^u_{-v}))$ and from $\mathcal{A}(f(U_{+v}))$ to $\mathcal{A}(f(U^u_{+v}))$. The remaining probability is transported arbitrarily.

First, let us fix the values of $c=c^u=\hat{c}$ and $d=d^u=\hat{d}$. Let $\mathcal{A}_{\hat{c},\hat{d}}(U)$ be the output distribution of Algorithm~\ref{alg:main} when $c=\hat{c}$ and $d=\hat{d}$ are sampled. For simplicity, we simply write $\Pr[\bar{v}=v|c=\hat{c},d=\hat{d}]$ (resp. $\Pr[\bar{v}^u=v|c^u=\hat{c},d^u=\hat{d}]$) by $\Pr[\bar{v}=v]$ (resp. $\Pr[\bar{v}^u=v]$).
Now, we have
\begin{align}
    &\EM(\mathcal{A}_{\hat{c},\hat{d}}(U)),\mathcal{A}_{\hat{c},\hat{d}}(U^u))\\
    &= \sum_{v\in U\setminus \{u\}}\min\left(\Pr[\bar{v}=v],\Pr[\bar{v}^u=v]\right)\left(\EM(\mathcal{A}(U_{-v}),\mathcal{A}(U^u_{-v}))+\EM(\mathcal{A}(U_{+v}),\mathcal{A}(U^u_{+v}))\right)\\
    &+ \sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\OPT(U).\label{eq:errorbarv}
\end{align}


Let us evaluate (\ref{eq:errorbarv}). The values $\Pr[\bar{v}=v]$ decreases by removing $u$ because of the following three reasons.
\begin{itemize}
    \item $u=v$ holds.
    \item $u$ is contained in all maximum chains that contains $v$. In this case, $r(v)>r^u(v)$ holds.
    \item $U_{\hat{d}}\subsetneq U_{\hat{d}}^u$ holds. In this case, the denominator $\sum_{v\in U_{\hat{d}}}\exp(r(v)/\hat{c})$ of the exponential mechanism increases.
\end{itemize}

The following lemma considers the case $u=v$ and it is clear.
\begin{lemma}
We have
\begin{align}
    \sum_{u\in U}\Pr[\bar{u}=u]=1.
\end{align}
\end{lemma}

The next lemma considers the second case.

\begin{lemma}
We have
\begin{align}
    \sum_{u\in U}\sum_{v\in U_{\hat{d}}\setminus \{u\}}\frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}\leq 2\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}
    &= \Pr[\bar{v}=v]\left(1-\frac{\exp(r^u(v)/\hat{c})}{\exp(r(v)/\hat{c})}\right)\\
    &= \Pr[\bar{v}=v]\left(1-\exp(-(r(v)-r^u(v))/\hat{c})\right)\\
    &\leq \Pr[\bar{v}=v]\cdot (r(v)-r^u(v))/\hat{c}.
\end{align}
Therefore, we have
\begin{align}
    \sum_{u\in U}\sum_{v\in U_{\hat{d}}\setminus \{u\}}\frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}
    &\leq \sum_{v\in U_{\hat{d}}}\Pr[\bar{v}=v]\sum_{u\in U\setminus \{v\}} c(r(v)-r^u(v))\\
    &\leq \sum_{v\in U_{\hat{d}}}\Pr[\bar{v}=v]\cdot r(v)/c\\
    &= \sum_{v\in U_{\hat{d}}}c\cdot \E[r(\bar{v})]\\
    &\leq \sum_{v\in U_{\hat{d}}}c\cdot \OPT(U)\\
    &\leq 2\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{proof}

The next lemma considers the last case.
\begin{lemma}
We have
\begin{align}
    &\sum_{u\in U}\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{v\in U_d\setminus \{u\}}\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d}^u}\exp(r^u(v')/\hat{c})}\right)\right)\mathrm{d}d
    \leq 4.
\end{align}
\end{lemma}
\begin{proof}
Since $\max\left(|U^u_{-v}|,|U^u_{+v}|\right)\geq \max\left(|U_{-v}|,|U_{+v}|\right)+1$, we have
\begin{align}
    &\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d}^u}\exp(r^u(v')/\hat{c})}\\
    &\leq \frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d+1}}\exp(r^u(v')/\hat{c})}\\
    &\leq \frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d+1}}\exp(r(v')/\hat{c})}.
\end{align}
By taking the expectation on $d$, we have
\begin{align}
    &\sum_{u\in U}\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{v\in U_d\setminus \{u\}}\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d}^u}\exp(r^u(v')/\hat{c})}\right)\right)\mathrm{d}d\\
    &\leq \sum_{u\in U}\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{v\in U_d\setminus \{u\}}\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d+1}}\exp(r(v')/\hat{c})}\right)\mathrm{d}d\\
    &=\sum_{u\in U}\frac{4}{|U|}\left(\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+1}\sum_{v\in U_d\setminus \{u\}}\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}\mathrm{d}d-\int_{\frac{3}{4}|U|}^{\frac{3}{4}|U|+1}\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}\mathrm{d}d\right)\\
    &\leq \sum_{u\in U}\frac{4}{|U|}\left(\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+1}\sum_{v\in U_d\setminus \{u\}}\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}\mathrm{d}d\right)\\
    &\leq \sum_{u\in U}\frac{4}{|U|}\left(\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+1}\mathrm{d}d\right)\\
    &= 4.
\end{align}
\end{proof}

Combine all.
\begin{lemma}
We have
\begin{align}
    \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\mathrm{d}d\leq 3\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    &\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\\
    &= \sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)+\sum_{u\in U}\max\left(0,\Pr[\bar{v}=u]-\Pr[\bar{v}^{u}=u]\right)\\
    &= \sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)+1.
\end{align}
Now, for $v\in U_{d}$ with $v\neq u$, we have
\begin{align}
    &\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\\
    &= \max\left(0,\frac{\exp(r(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}-\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}^u}\exp(r^u(v')/\hat{c})}\right)\\
    &\leq \frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}
    +\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{\hat{d}}^u}\exp(r^u(v')/\hat{c})}\right)\right).
\end{align}
Now, we have
\begin{align}
    &\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\mathrm{d}d\\
    &= \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\mathrm{d}d+1\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U\setminus u}\frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}\mathrm{d}d\\
    &+ \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{\hat{d}}^u}\exp(r^u(v')/\hat{c})}\right)\right)\mathrm{d}d+1\\
    &\leq 2\epsilon^{-1}\log(|U|\epsilon^{-1})+4+1\leq 3\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{proof}

Now let us evaluate the impact to sample $c$ and $d$.
First, we bound the impact to the average sensitivity of choosing parameters from uniform distribution.

\begin{lemma}
Let $t>0$ be a real number and $p$ (resp. $p^u$) be a parameter in an algorithm for the instance $U$ (resp. $U^u$), sampled from the uniform distribution on $[B,(1+t)B]$ (resp. $[B^u,(1+t)B^u]$). Then, we have
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\int_{B}^{(1+t)B}\frac{1}{tB}\sum_{u\in U}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}+\frac{1+t}{t}\cdot \sum_{u\in U}\left|1-\frac{B^u}{B}\right|.
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    &\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \int_{[B,(1+t)B]\cap [B^u,(1+t)B^u]}\min\left(\frac{1}{tB},\frac{1}{tB^u}\right)\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}\label{eq:uniform1}\\ 
    &\quad \quad + \int_{[B,(1+t)B]\cap [B^u,(1+t)B^u]}\max\left(0,\frac{1}{tB}-\frac{1}{tB^u}\right)|U|\mathrm{d}\hat{p} + \int_{[B,(1+t)B]\setminus [B^u,(1+t)B^u]}\frac{1}{tB}|U|\mathrm{d}\hat{p}. \label{eq:uniform2}
\end{align}
Now, we have
\begin{align}
    (\ref{eq:uniform1})
    &\leq \int_{B}^{(1+t)B}\frac{1}{tB}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}.
    %\\
    %&\leq \sup_{\hat{p}\in [B,(1+t)B]}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right).
\end{align}
Now, if $B^u\leq B$, we have
\begin{align}
    (\ref{eq:uniform2})
    &\leq 0 + \int_{(1+t)B^u}^{(1+t)B}\frac{1}{tB}|U|\mathrm{d}\hat{p}\\
    &=\frac{(1+t)(B-B^u)}{tB}|U|=\frac{1+t}{t}\cdot \left|1-\frac{B^u}{B}\right||U|.
\end{align}
Otherwise, we have
\begin{align}
    (\ref{eq:uniform2})
    &\leq \int_{B}^{(1+t)B}\left(\frac{1}{tB}-\frac{1}{tB^u}\right)|U|\mathrm{d}\hat{p} + \int_{B}^{B^u}\frac{1}{tB}|U|\mathrm{d}\hat{p}\\
    &=\left(\left(\frac{1}{tB}-\frac{1}{tB^u}\right)tB+\frac{B^u-B}{tB}\right)|U|\\
    &=\left(\frac{1}{B^u}+\frac{1}{tB}\right)(B^u-B)|U|\leq \frac{1+t}{t}\cdot \left|1-\frac{B^u}{B}\right||U|.
\end{align}
Therefore, we have
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\sum_{u\in U}\int_{B}^{(1+t)B}\frac{1}{tB}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}+\frac{1}{|U|}\sum_{u\in U}\frac{1+t}{t}\cdot \left|1-\frac{B^u}{B}\right||U|\\
    &= \frac{1}{|U|}\int_{B}^{(1+t)B}\frac{1}{tB}\sum_{u\in U}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}+\frac{1+t}{t}\cdot \sum_{u\in U}\left|1-\frac{B^u}{B}\right|.
\end{align}
\end{proof}

We evaluate the impact of sampling $\hat{c}$.

\begin{lemma}
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq\frac{1}{|U|}\sup_{\hat{c}\in [B,2B]}\sum_{u\in U}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^u=\hat{c}}(U^u)\right)\mathrm{d}\hat{c}+6\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}
\begin{proof}
Let $B=\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}$ and $B^u=\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}$.
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\int_{B}^{2B}\frac{1}{2B}\sum_{u\in U}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^u=\hat{c}}(U^u)\right)\mathrm{d}\hat{c}+2\cdot \sum_{u\in U}\left|1-\frac{B^u}{B}\right|\\
    &\leq\frac{1}{|U|}\sup_{\hat{c}\in [B,2B]}\sum_{u\in U}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^u=\hat{c}}(U^u)\right)\mathrm{d}\hat{c}+\frac{2}{B}\cdot \sum_{u\in U}\left|B-B^u\right|.
\end{align}
Now,
\begin{align}
    \frac{1}{B}\left|B-B^u\right|
    &=\frac{1}{B}\left|\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}\right|\\
    &=\frac{1}{B}\left|\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}\right|
    +\frac{1}{B}\left|\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}\right|
\end{align}
Now, 
\begin{align}
    \sum_{u\in U}\frac{1}{B}\left|\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}\right|
    &= \sum_{u\in U}\frac{\log(|U|\epsilon^{-1})}{\log((|U|-1)\epsilon^{-1})}\left(1-\frac{\OPT(U^u)}{\OPT(U)}\right)\\
    &\leq 2\cdot \frac{1}{\OPT(U)}\sum_{u\in U}(\OPT(U)-\OPT(U^u))\\
    &\leq 2.
\end{align}
\end{proof}
And,
\begin{align}
    \sum_{u\in U}\frac{1}{B}\left|\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}\right|
    &= \sum_{u\in U}\log(|U|\epsilon^{-1})\left(\frac{1}{\log(|U|-1)}-\frac{1}{\log(|U|)}\right)\\
    &\leq |U|\log(|U|\epsilon^{-1})\cdot \frac{2}{|U|}\\
    &\leq 2\log(|U|\epsilon^{-1}).
\end{align}


We evaluate the impact of sampling $d$.
\begin{lemma}

\end{lemma}
\begin{proof}
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\frac{4}{|U|}\sum_{u\in U}\EM\left(\mathcal{A}|_{d=\hat{d}}(U),\mathcal{A}|_{d^u=\hat{d}}(U^u)\right)\mathrm{d}\hat{d}+3\cdot \sum_{u\in U}\left|1-\frac{\frac{1}{2}(|U|-1)}{\frac{1}{2}|U|}\right|\\
    &= \frac{1}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\frac{4}{|U|}\sum_{u\in U}\EM\left(\mathcal{A}|_{d=\hat{d}}(U),\mathcal{A}|_{d^u=\hat{d}}(U^u)\right)\mathrm{d}\hat{d}+3.
\end{align}
\end{proof}



Now we prove the following lemma by induction on $|U|$.
\begin{lemma}
\begin{align}
    \frac{1}{|U|}\sum_{u\in U}\EM[\mathcal{A}(U),\mathcal{A}(U^u)]\leq 4\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}

\begin{lemma}
Assume the induction hypothesis holds. Then, we have
\begin{align}
    &\sum_{u\in U}\sum_{v\in U_{d}\setminus \{u\}}\Pr[\bar{v}=v]\left(\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))+\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))\right)\\
    &\leq hoge.
\end{align}
\end{lemma}
\begin{proof}
Let us fix $u\in U$ and $v\in U_{d}\setminus \{u\}$. If $u$ is not in neither $U_{-v}$ nor $U_{+v}$, we have
\begin{align}
    \EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))=\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))=0.
\end{align}
Assume $u$ is in either $U_{-v}$ or $U_{+v}$. Without loss of generality, we can assume $u\in U_{-v}$ and
\begin{align}
    \EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))=0.
\end{align}
Therefore, we have
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\left(\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))+\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))\right)\\
    &= \frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))\\
    &\leq \frac{3}{4}\cdot 4\epsilon^{-1}\log\left(\frac{3}{4}|U|\epsilon^{-1}\right).
\end{align}
\end{proof}

Combine all.

\begin{lemma}
Induction.
\end{lemma}
\begin{proof}
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}_{\hat{c},\hat{d}}(U)),\mathcal{A}_{\hat{c},\hat{d}}(U^u))+7\log(|U|\epsilon^{-1})\\
    &\leq \frac{1}{|U|}\sum_{u\in U}\sum_{v\in U\setminus \{u\}}\min\left(\Pr[\bar{v}=v],\Pr[\bar{v}^u=v]\right)\left(\EM(\mathcal{A}(U_{-v}),\mathcal{A}(U^u_{-v}))+\EM(\mathcal{A}(U_{+v}),\mathcal{A}(U^u_{+v}))\right)\\
    &+ \frac{1}{|U|}\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\OPT(U)+7\log(|U|\epsilon^{-1})\\
    &\leq \frac{3}{4}\cdot 4\epsilon^{-1}\log\left(\frac{3}{4}|U|\epsilon^{-1}\right)+3\epsilon^{-1}\log(|U|\epsilon^{-1})+7\log(|U|\epsilon^{-1})\\
    &\leq 4\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right).
\end{align}
\end{proof}

\begin{lemma}
There is an algorithm to maximum weight chain problem on DAG with approximation ratio $1-\epsilon$ and average sensitivity $O(\epsilon^{-1}\log |V|(\log |V|+\log \epsilon^{-1}))$.
\end{lemma}
\begin{proof}
Let $B=\frac{7\log(|V|)}{\epsilon}$. First, we sample $\epsilon^{-1}$ in algorithm from uniform distribution over $[B,2B]$ and apply the algorithm. Then, the approximation ratio is at most $1-\epsilon$. The average sensitivity is bounded as
\begin{align}
    &\frac{1}{|V|}\sum_{u\in V}\EM[\mathcal{A}(V),\mathcal{A}(V^u)]\\
    &\frac{1}{|V|}\sum_{u\in V}\int_{B}^{2B}\frac{1}{B}\EM(\mathcal{A}_{b^{-1}}(V),\mathcal{A}_{b^{-1}}(V^u))\mathrm{d}b
    +\sum_{u\in V}2\cdot \left|1-\frac{\log(|V|)}{\log(|V|-1)}\right|\\
    &\leq \frac{1}{|V|}\sum_{u\in V}\sup_{b^{-1}\in [B,2B]}\left(\EM(\mathcal{A}_{b^{-1}}(V),\mathcal{A}_{b^{-1}}(V^u))\right)
    +2\cdot \sum_{u\in V}\left|1-\frac{\log(|V|-1)}{\log(|V|)}\right|\\
    &\leq 4\cdot 14\log |V|\epsilon^{-1}\log\left(|V|\cdot 7\log(|V|)\epsilon^{-1}\right)
    +2\cdot \sum_{u\in V}\frac{2}{|V|}\\
    &\leq 56\epsilon^{-1}\cdot \log |V| \cdot \left(\log(7|V|)+\log \log |V|+\log \epsilon^{-1}\right)+4\\
    &\leq O(\epsilon^{-1}\log |V|(\log |V|+\log \epsilon^{-1})).
\end{align}
\end{proof}

==> old/furuino.tex <==
\section{DAG Longest Chain}

Let $G=(V,E)$ be a transitive directed acyclic graph. %For a vertex $v\in V$, let $(-\infty, v)$ be the set of vertices from which there is an edge to $v$, and $(v,\infty)$ be the set of vertices to which there is an edge from $v$. For two vertices $u,v\in V$, let $(u,v)=(u,\infty)\cap (-\infty,v)$. For simplicity, we write $V=(-\infty, \infty)$.

A vertex $v\in U$ is \emph{central} in $U$ if $|U_{-v}|\leq \frac{|U|}{2}$ and $|U_{+v}|\leq \frac{|U|}{2}$.

\begin{algorithm}[t!]
\caption{Less-sensitive Maximum Weight Chain $f(U)$}
\begin{algorithmic}[1]\label{alg:main}
\STATE Sample $c$ from the uniform distribution over $\left[\frac{\epsilon \OPT(U)}{\log(|U|\epsilon^{-1})},2\cdot \frac{\epsilon \OPT(U)}{\log(|U|\epsilon^{-1})} \right]$
\STATE Sample $d$ from the uniform distribution over $\left[\frac{1}{2}|U|,\frac{3}{4}|U|\right]$
\IF{$U=\emptyset$}
    \RETURN $\emptyset$
\ENDIF
\FOR{$v\in U$}
    \STATE Let $r(v)$ be the maximum weight of a chain that contains $v$
\ENDFOR
\STATE Let $U_d$ be the set of the vertices with $\max\left(|U_{-v}|,|U_{+v}|\right)\leq d$
\STATE Sample $\bar{v}\in U_d$ with probability proportional to $\exp(r(\bar{v})/c)$
\RETURN $f(U_{-\bar{v}})\cup \{\bar{v}\}\cup f(U_{+\bar{v}})$
\end{algorithmic}
\end{algorithm}

The answer is $f(V)$.

\begin{lemma}
There is a central vertex in $U$ with $r(v)=\OPT(U)$. Particularly, $\max_{v\in U_d}r(v)=\OPT(U)$.
\end{lemma}
\begin{proof}
Let $C=(v_1,\dots, v_k)$ be a maximal chain that attains $\OPT(U)$. Let $v_i$ be the last vertex with $|U_{-v}|\leq \frac{|U|}{2}$. We prove that $|U_{+v_i}|\leq \frac{|U|}{2}$.

If $i=k$, $|U_{+v_i}|=0$ because $C$ is maximal. Otherwise, we have
\begin{align}
    |U_{+v_i}|&=|U_{+v_i}\setminus U_{-v_{i+1}}|+|U_{+v_i}\cap U_{-v_{i+1}}|\\
    &=|U_{+v_i}\setminus U_{-v_{i+1}}|\\
    &\leq |U\setminus U_{-v_{i+1}}|\leq \frac{|U|}{2},
\end{align}
where the second equality is from $|U_{+v_i}\cap U_{-v_{i+1}}|=0$ that is from the maximality of $C$ and the last inequality is from the definition of $i$.
\end{proof}


First we analyze the approximation factor. First we analyze the loss by the exponential mechanism.

\begin{lemma}
We have 
\begin{align}
    \E[r(\bar{v})]\geq (1-2\epsilon) \OPT(U).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    \Pr[r(\bar{v}) \leq (1-\epsilon)\OPT(U)]
    &= \frac{\sum_{v\in U_d, r(v)\leq (1-\epsilon) \OPT(U)}\exp(r(v)/c)}{\sum_{v\in U_d}\exp(r(v)/c)}\\
    &\leq \frac{|U_d|\exp((1-\epsilon)\OPT(U)/c)}{\sum_{v\in U_d}\exp(r(v)/c)}\\
    &\leq \frac{|U_d|\exp((1-\epsilon)\OPT(U)/c)}{\exp(\OPT(U)/c)}\\
    &= |U_d|\exp(-\epsilon \cdot \OPT(U)/c)\\
    &= |U_d|\cdot \frac{\epsilon}{|U|}\\
    &\leq \epsilon.
\end{align}

Therefore, we have
\begin{align}
    \E[r(\bar{v})]
    &\geq (1-\epsilon)(1-\epsilon)\OPT(U)\\
    &\geq (1-2\epsilon)\OPT(U).
\end{align}
\end{proof}


Next, we analyze the loss by the recursion.

\begin{lemma}
We have
\begin{align}
    \E\left[w(f(U))\right]\geq (1-7\epsilon\log |U|)\OPT(U).
\end{align}
\end{lemma}
\begin{proof}
We prove by induction on $|U|$. If $|U|=1$, the statement is clear.
Now, we have
\begin{align}
    \E\left[w(f(U))\right]
    &= \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left(\E\left[w(f(U_{-v}))\right]+\E\left[w(f(U_{+v}))\right]\right)\right]+1\\
    &\geq \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left((1-7\epsilon \log |U_{-v}|)\OPT(U_{-v})+(1-7\epsilon \log |U_{+v}|)\OPT(U_{+v})\right)\right]+1\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left(\OPT(U_{-v})+\OPT(U_{+v})\right)\right]+1\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]r(v)\right]\\
    &= \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[r(\bar{v})\right]\\
    &\geq \left(1-7\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right)(1-2\epsilon)\OPT(U)\\
    &\geq \left(1-7\epsilon\log \left(\frac{3}{4}\OPT(U)\right)-2\epsilon \right)\OPT(U)\\
    &\geq (1-7\epsilon\log \OPT(U))\OPT(U).
\end{align}
\end{proof}


Next we analyze the sensitivity. We denote $r(v)$ in the Algorithm~\ref{alg:main} on the instance $U\setminus \{u\}$ by $r^u(v)$.

To evaluate the earth mover's distance, we recursively transport the probability. We transport the probability so that the case of same choices of $c$, $d$, and $\bar{v}$ correspond to each other. For these cases, We recursively transport the probability from $\mathcal{A}(f(U_{-v}))$ to $\mathcal{A}(f(U^u_{-v}))$ and from $\mathcal{A}(f(U_{+v}))$ to $\mathcal{A}(f(U^u_{+v}))$. The remaining probability is transported arbitrarily.

First, let us fix the values of $c=c^u=\hat{c}$ and $d=d^u=\hat{d}$. Let $\mathcal{A}_{\hat{c},\hat{d}}(U)$ be the output distribution of Algorithm~\ref{alg:main} when $c=\hat{c}$ and $d=\hat{d}$ are sampled. For simplicity, we simply write $\Pr[\bar{v}=v|c=\hat{c},d=\hat{d}]$ (resp. $\Pr[\bar{v}^u=v|c^u=\hat{c},d^u=\hat{d}]$) by $\Pr[\bar{v}=v]$ (resp. $\Pr[\bar{v}^u=v]$).
Now, we have
\begin{align}
    &\EM(\mathcal{A}_{\hat{c},\hat{d}}(U)),\mathcal{A}_{\hat{c},\hat{d}}(U^u))\\
    &= \sum_{v\in U\setminus \{u\}}\min\left(\Pr[\bar{v}=v],\Pr[\bar{v}^u=v]\right)\left(\EM(\mathcal{A}(U_{-v}),\mathcal{A}(U^u_{-v}))+\EM(\mathcal{A}(U_{+v}),\mathcal{A}(U^u_{+v}))\right)\\
    &+ \sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\OPT(U).\label{eq:errorbarv}
\end{align}


Let us evaluate (\ref{eq:errorbarv}). The values $\Pr[\bar{v}=v]$ decreases by removing $u$ because of the following three reasons.
\begin{itemize}
    \item $u=v$ holds.
    \item $u$ is contained in all maximum chains that contains $v$. In this case, $r(v)>r^u(v)$ holds.
    \item $U_{\hat{d}}\subsetneq U_{\hat{d}}^u$ holds. In this case, the denominator $\sum_{v\in U_{\hat{d}}}\exp(r(v)/\hat{c})$ of the exponential mechanism increases.
\end{itemize}

The following lemma considers the case $u=v$ and it is clear.
\begin{lemma}
We have
\begin{align}
    \sum_{u\in U}\Pr[\bar{u}=u]=1.
\end{align}
\end{lemma}

The next lemma considers the second case.

\begin{lemma}
We have
\begin{align}
    \sum_{u\in U}\sum_{v\in U_{\hat{d}}\setminus \{u\}}\frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}\leq 2\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}
    &= \Pr[\bar{v}=v]\left(1-\frac{\exp(r^u(v)/\hat{c})}{\exp(r(v)/\hat{c})}\right)\\
    &= \Pr[\bar{v}=v]\left(1-\exp(-(r(v)-r^u(v))/\hat{c})\right)\\
    &\leq \Pr[\bar{v}=v]\cdot (r(v)-r^u(v))/\hat{c}.
\end{align}
Therefore, we have
\begin{align}
    \sum_{u\in U}\sum_{v\in U_{\hat{d}}\setminus \{u\}}\frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}
    &\leq \sum_{v\in U_{\hat{d}}}\Pr[\bar{v}=v]\sum_{u\in U\setminus \{v\}} c(r(v)-r^u(v))\\
    &\leq \sum_{v\in U_{\hat{d}}}\Pr[\bar{v}=v]\cdot r(v)/c\\
    &= \sum_{v\in U_{\hat{d}}}c\cdot \E[r(\bar{v})]\\
    &\leq \sum_{v\in U_{\hat{d}}}c\cdot \OPT(U)\\
    &\leq 2\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{proof}

The next lemma considers the last case.
\begin{lemma}
We have
\begin{align}
    &\sum_{u\in U}\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{v\in U_d\setminus \{u\}}\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d}^u}\exp(r^u(v')/\hat{c})}\right)\right)\mathrm{d}d
    \leq 4.
\end{align}
\end{lemma}
\begin{proof}
Since $\max\left(|U^u_{-v}|,|U^u_{+v}|\right)\geq \max\left(|U_{-v}|,|U_{+v}|\right)+1$, we have
\begin{align}
    &\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d}^u}\exp(r^u(v')/\hat{c})}\\
    &\leq \frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d+1}}\exp(r^u(v')/\hat{c})}\\
    &\leq \frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d+1}}\exp(r(v')/\hat{c})}.
\end{align}
By taking the expectation on $d$, we have
\begin{align}
    &\sum_{u\in U}\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{v\in U_d\setminus \{u\}}\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d}^u}\exp(r^u(v')/\hat{c})}\right)\right)\mathrm{d}d\\
    &\leq \sum_{u\in U}\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{v\in U_d\setminus \{u\}}\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{d+1}}\exp(r(v')/\hat{c})}\right)\mathrm{d}d\\
    &=\sum_{u\in U}\frac{4}{|U|}\left(\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+1}\sum_{v\in U_d\setminus \{u\}}\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}\mathrm{d}d-\int_{\frac{3}{4}|U|}^{\frac{3}{4}|U|+1}\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}\mathrm{d}d\right)\\
    &\leq \sum_{u\in U}\frac{4}{|U|}\left(\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+1}\sum_{v\in U_d\setminus \{u\}}\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{d}}\exp(r(v')/\hat{c})}\mathrm{d}d\right)\\
    &\leq \sum_{u\in U}\frac{4}{|U|}\left(\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+1}\mathrm{d}d\right)\\
    &= 4.
\end{align}
\end{proof}

Combine all.
\begin{lemma}
We have
\begin{align}
    \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\mathrm{d}d\leq 3\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    &\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\\
    &= \sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)+\sum_{u\in U}\max\left(0,\Pr[\bar{v}=u]-\Pr[\bar{v}^{u}=u]\right)\\
    &= \sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)+1.
\end{align}
Now, for $v\in U_{d}$ with $v\neq u$, we have
\begin{align}
    &\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\\
    &= \max\left(0,\frac{\exp(r(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}-\frac{\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}^u}\exp(r^u(v')/\hat{c})}\right)\\
    &\leq \frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}
    +\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{\hat{d}}^u}\exp(r^u(v')/\hat{c})}\right)\right).
\end{align}
Now, we have
\begin{align}
    &\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\mathrm{d}d\\
    &= \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\mathrm{d}d+1\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U\setminus u}\frac{\exp(r(v)/\hat{c})-\exp(r^u(v)/\hat{c})}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}\mathrm{d}d\\
    &+ \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\sum_{u\in U}\sum_{v\in U\setminus u}\max\left(0,\exp(r^u(v)/\hat{c})\left(\frac{1}{\sum_{v'\in U_{\hat{d}}}\exp(r(v')/\hat{c})}-\frac{1}{\sum_{v'\in U_{\hat{d}}^u}\exp(r^u(v')/\hat{c})}\right)\right)\mathrm{d}d+1\\
    &\leq 2\epsilon^{-1}\log(|U|\epsilon^{-1})+4+1\leq 3\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{proof}

Now let us evaluate the impact to sample $c$ and $d$.
First, we bound the impact to the average sensitivity of choosing parameters from uniform distribution.

\begin{lemma}
Let $t>0$ be a real number and $p$ (resp. $p^u$) be a parameter in an algorithm for the instance $U$ (resp. $U^u$), sampled from the uniform distribution on $[B,(1+t)B]$ (resp. $[B^u,(1+t)B^u]$). Then, we have
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\int_{B}^{(1+t)B}\frac{1}{tB}\sum_{u\in U}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}+\frac{1+t}{t}\cdot \sum_{u\in U}\left|1-\frac{B^u}{B}\right|.
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    &\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \int_{[B,(1+t)B]\cap [B^u,(1+t)B^u]}\min\left(\frac{1}{tB},\frac{1}{tB^u}\right)\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}\label{eq:uniform1}\\ 
    &\quad \quad + \int_{[B,(1+t)B]\cap [B^u,(1+t)B^u]}\max\left(0,\frac{1}{tB}-\frac{1}{tB^u}\right)|U|\mathrm{d}\hat{p} + \int_{[B,(1+t)B]\setminus [B^u,(1+t)B^u]}\frac{1}{tB}|U|\mathrm{d}\hat{p}. \label{eq:uniform2}
\end{align}
Now, we have
\begin{align}
    (\ref{eq:uniform1})
    &\leq \int_{B}^{(1+t)B}\frac{1}{tB}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}.
    %\\
    %&\leq \sup_{\hat{p}\in [B,(1+t)B]}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right).
\end{align}
Now, if $B^u\leq B$, we have
\begin{align}
    (\ref{eq:uniform2})
    &\leq 0 + \int_{(1+t)B^u}^{(1+t)B}\frac{1}{tB}|U|\mathrm{d}\hat{p}\\
    &=\frac{(1+t)(B-B^u)}{tB}|U|=\frac{1+t}{t}\cdot \left|1-\frac{B^u}{B}\right||U|.
\end{align}
Otherwise, we have
\begin{align}
    (\ref{eq:uniform2})
    &\leq \int_{B}^{(1+t)B}\left(\frac{1}{tB}-\frac{1}{tB^u}\right)|U|\mathrm{d}\hat{p} + \int_{B}^{B^u}\frac{1}{tB}|U|\mathrm{d}\hat{p}\\
    &=\left(\left(\frac{1}{tB}-\frac{1}{tB^u}\right)tB+\frac{B^u-B}{tB}\right)|U|\\
    &=\left(\frac{1}{B^u}+\frac{1}{tB}\right)(B^u-B)|U|\leq \frac{1+t}{t}\cdot \left|1-\frac{B^u}{B}\right||U|.
\end{align}
Therefore, we have
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\sum_{u\in U}\int_{B}^{(1+t)B}\frac{1}{tB}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}+\frac{1}{|U|}\sum_{u\in U}\frac{1+t}{t}\cdot \left|1-\frac{B^u}{B}\right||U|\\
    &= \frac{1}{|U|}\int_{B}^{(1+t)B}\frac{1}{tB}\sum_{u\in U}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^u=\hat{p}}(U^u)\right)\mathrm{d}\hat{p}+\frac{1+t}{t}\cdot \sum_{u\in U}\left|1-\frac{B^u}{B}\right|.
\end{align}
\end{proof}

We evaluate the impact of sampling $\hat{c}$.

\begin{lemma}
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq\frac{1}{|U|}\sup_{\hat{c}\in [B,2B]}\sum_{u\in U}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^u=\hat{c}}(U^u)\right)\mathrm{d}\hat{c}+6\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}
\begin{proof}
Let $B=\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}$ and $B^u=\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}$.
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\int_{B}^{2B}\frac{1}{2B}\sum_{u\in U}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^u=\hat{c}}(U^u)\right)\mathrm{d}\hat{c}+2\cdot \sum_{u\in U}\left|1-\frac{B^u}{B}\right|\\
    &\leq\frac{1}{|U|}\sup_{\hat{c}\in [B,2B]}\sum_{u\in U}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^u=\hat{c}}(U^u)\right)\mathrm{d}\hat{c}+\frac{2}{B}\cdot \sum_{u\in U}\left|B-B^u\right|.
\end{align}
Now,
\begin{align}
    \frac{1}{B}\left|B-B^u\right|
    &=\frac{1}{B}\left|\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}\right|\\
    &=\frac{1}{B}\left|\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}\right|
    +\frac{1}{B}\left|\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}\right|
\end{align}
Now, 
\begin{align}
    \sum_{u\in U}\frac{1}{B}\left|\frac{\epsilon\OPT(U^u)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}\right|
    &= \sum_{u\in U}\frac{\log(|U|\epsilon^{-1})}{\log((|U|-1)\epsilon^{-1})}\left(1-\frac{\OPT(U^u)}{\OPT(U)}\right)\\
    &\leq 2\cdot \frac{1}{\OPT(U)}\sum_{u\in U}(\OPT(U)-\OPT(U^u))\\
    &\leq 2.
\end{align}
\end{proof}
And,
\begin{align}
    \sum_{u\in U}\frac{1}{B}\left|\frac{\epsilon\OPT(U)}{\log(|U^u|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U|\epsilon^{-1})}\right|
    &= \sum_{u\in U}\log(|U|\epsilon^{-1})\left(\frac{1}{\log(|U|-1)}-\frac{1}{\log(|U|)}\right)\\
    &\leq |U|\log(|U|\epsilon^{-1})\cdot \frac{2}{|U|}\\
    &\leq 2\log(|U|\epsilon^{-1}).
\end{align}


We evaluate the impact of sampling $d$.
\begin{lemma}

\end{lemma}
\begin{proof}
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\frac{4}{|U|}\sum_{u\in U}\EM\left(\mathcal{A}|_{d=\hat{d}}(U),\mathcal{A}|_{d^u=\hat{d}}(U^u)\right)\mathrm{d}\hat{d}+3\cdot \sum_{u\in U}\left|1-\frac{\frac{1}{2}(|U|-1)}{\frac{1}{2}|U|}\right|\\
    &= \frac{1}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\frac{4}{|U|}\sum_{u\in U}\EM\left(\mathcal{A}|_{d=\hat{d}}(U),\mathcal{A}|_{d^u=\hat{d}}(U^u)\right)\mathrm{d}\hat{d}+3.
\end{align}
\end{proof}



Now we prove the following lemma by induction on $|U|$.
\begin{lemma}
\begin{align}
    \frac{1}{|U|}\sum_{u\in U}\EM[\mathcal{A}(U),\mathcal{A}(U^u)]\leq 4\epsilon^{-1}\log(|U|\epsilon^{-1}).
\end{align}
\end{lemma}

\begin{lemma}
Assume the induction hypothesis holds. Then, we have
\begin{align}
    &\sum_{u\in U}\sum_{v\in U_{d}\setminus \{u\}}\Pr[\bar{v}=v]\left(\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))+\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))\right)\\
    &\leq hoge.
\end{align}
\end{lemma}
\begin{proof}
Let us fix $u\in U$ and $v\in U_{d}\setminus \{u\}$. If $u$ is not in neither $U_{-v}$ nor $U_{+v}$, we have
\begin{align}
    \EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))=\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))=0.
\end{align}
Assume $u$ is in either $U_{-v}$ or $U_{+v}$. Without loss of generality, we can assume $u\in U_{-v}$ and
\begin{align}
    \EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))=0.
\end{align}
Therefore, we have
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\left(\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))+\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))\right)\\
    &= \frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))\\
    &\leq \frac{3}{4}\cdot 4\epsilon^{-1}\log\left(\frac{3}{4}|U|\epsilon^{-1}\right).
\end{align}
\end{proof}

Combine all.

\begin{lemma}
Induction.
\end{lemma}
\begin{proof}
\begin{align}
    &\frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}(U),\mathcal{A}(U^u))\\
    &\leq \frac{1}{|U|}\sum_{u\in U}\EM(\mathcal{A}_{\hat{c},\hat{d}}(U)),\mathcal{A}_{\hat{c},\hat{d}}(U^u))+7\log(|U|\epsilon^{-1})\\
    &\leq \frac{1}{|U|}\sum_{u\in U}\sum_{v\in U\setminus \{u\}}\min\left(\Pr[\bar{v}=v],\Pr[\bar{v}^u=v]\right)\left(\EM(\mathcal{A}(U_{-v}),\mathcal{A}(U^u_{-v}))+\EM(\mathcal{A}(U_{+v}),\mathcal{A}(U^u_{+v}))\right)\\
    &+ \frac{1}{|U|}\sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\OPT(U)+7\log(|U|\epsilon^{-1})\\
    &\leq \frac{3}{4}\cdot 4\epsilon^{-1}\log\left(\frac{3}{4}|U|\epsilon^{-1}\right)+3\epsilon^{-1}\log(|U|\epsilon^{-1})+7\log(|U|\epsilon^{-1})\\
    &\leq 4\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right).
\end{align}
\end{proof}

\begin{lemma}
There is an algorithm to maximum weight chain problem on DAG with approximation ratio $1-\epsilon$ and average sensitivity $O(\epsilon^{-1}\log |V|(\log |V|+\log \epsilon^{-1}))$.
\end{lemma}
\begin{proof}
Let $B=\frac{7\log(|V|)}{\epsilon}$. First, we sample $\epsilon^{-1}$ in algorithm from uniform distribution over $[B,2B]$ and apply the algorithm. Then, the approximation ratio is at most $1-\epsilon$. The average sensitivity is bounded as
\begin{align}
    &\frac{1}{|V|}\sum_{u\in V}\EM[\mathcal{A}(V),\mathcal{A}(V^u)]\\
    &\frac{1}{|V|}\sum_{u\in V}\int_{B}^{2B}\frac{1}{B}\EM(\mathcal{A}_{b^{-1}}(V),\mathcal{A}_{b^{-1}}(V^u))\mathrm{d}b
    +\sum_{u\in V}2\cdot \left|1-\frac{\log(|V|)}{\log(|V|-1)}\right|\\
    &\leq \frac{1}{|V|}\sum_{u\in V}\sup_{b^{-1}\in [B,2B]}\left(\EM(\mathcal{A}_{b^{-1}}(V),\mathcal{A}_{b^{-1}}(V^u))\right)
    +2\cdot \sum_{u\in V}\left|1-\frac{\log(|V|-1)}{\log(|V|)}\right|\\
    &\leq 4\cdot 14\log |V|\epsilon^{-1}\log\left(|V|\cdot 7\log(|V|)\epsilon^{-1}\right)
    +2\cdot \sum_{u\in V}\frac{2}{|V|}\\
    &\leq 56\epsilon^{-1}\cdot \log |V| \cdot \left(\log(7|V|)+\log \log |V|+\log \epsilon^{-1}\right)+4\\
    &\leq O(\epsilon^{-1}\log |V|(\log |V|+\log \epsilon^{-1})).
\end{align}
\end{proof}

==> old/honmono2.tex <==
%!TEX root=./main.tex

\section{DAG Longest Chain}

Let $G=(V,E)$ be a transitive directed acyclic graph. Let $S_1,\dots, S_n$ be antichains of $G$ such that each element of $v$ is contained in at least one and at most $K$ of them. Note that, since a chain cannot contain two vertices from the same $S_i$, the size of any feasible solution is at most $n$. The average sensitivity of an algorithm $\mathcal{A}$ is defined by
\begin{align}
    \frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(V), \mathcal{A}(V\setminus S_i)).
\end{align}


\begin{algorithm}[t!]
\caption{Less-sensitive Maximum Weight Chain $f(U)$}\label{alg:main}
\Procedure{\emph{\Call{InsensitiveMaxWeightChain}{$U$}}}{
    Sample $c$ from the uniform distribution over $\left[\frac{\epsilon \OPT(U)}{\log\left(|U|\epsilon^{-1}\right)},2\cdot \frac{\epsilon \OPT(U)}{\log\left(|U|\epsilon^{-1}\right)} \right]$\;
    Sample $d$ from the uniform distribution over $\left[\frac{1}{2}|U|,\frac{3}{4}|U|\right]$\;
    \If{$U=\emptyset$}{
        \Return $\emptyset$\;
    }
    \For{$v\in U$}{
        Let $r(v)$ be the maximum weight of a chain that contains $v$\;
    }
    Let $U_d$ be the set of the vertices with $\max\left(|U_{-v}|,|U_{+v}|\right)\leq d$\;
    Sample $\bar{v}\in U_d$ with probability proportional to $\exp(r(\bar{v})/c)$\;
    \Return \Call{InsensitiveMaxWeightChain}{$U_{-\bar{v}}$} $\cup$ $\{\bar{v}\}$ $\cup$ \Call{InsensitiveMaxWeightChain}{$U_{+\bar{v}}$}\;
}
\end{algorithm}

A vertex $v\in U$ is \emph{central} in $U$ if $|U_{-v}|\leq \frac{|U|}{2}$ and $|U_{+v}|\leq \frac{|U|}{2}$. We begin by the following lemma.

\begin{lemma}
There is a central vertex in $U$ with $r(v)=\OPT(U)$. Particularly, $\max_{v\in U_d}r(v)=\OPT(U)$.
\end{lemma}
\begin{proof}
Let $C=(v_1,\dots, v_k)$ be a maximal chain that attains $\OPT(U)$. Let $v_i$ be the last vertex with $|U_{-v}|\leq \frac{|U|}{2}$. We prove that $|U_{+v_i}|\leq \frac{|U|}{2}$.

If $i=k$, $|U_{+v_i}|=0$ because $C$ is maximal. Otherwise, we have
\begin{align}
    |U_{+v_i}|&=|U_{+v_i}\setminus U_{-v_{i+1}}|+|U_{+v_i}\cap U_{-v_{i+1}}|\\
    &=|U_{+v_i}\setminus U_{-v_{i+1}}|\\
    &\leq |U\setminus U_{-v_{i+1}}|\leq \frac{|U|}{2},
\end{align}
where the second equality is from $|U_{+v_i}\cap U_{-v_{i+1}}|=0$ that is from the maximality of $C$ and the last inequality is from the definition of $i$.
\end{proof}

The next lemma is useful.

\begin{lemma}\label{lem:sumdiff}
We have
\begin{align}
    \sum_{i=1}^{n}(\OPT(U)-\OPT(U^i))\leq K\OPT(U).
\end{align}
\end{lemma}
\begin{proof}
Let $X$ be a solution that attains $U$. Then, we have
\begin{align}
    \sum_{i=1}^{n}(\OPT(U)-\OPT(U^i))
    &\leq \sum_{i=1}^{n}\left(w(X)-w(X\setminus S_i)\right)\\
    &= \sum_{i=1}^{n}w(X\cap S_i)\leq K\cdot w(X) = K\OPT(U),
\end{align}
where the first inequality is from the fact that $X\setminus S_i$ is a feasible solution and the second inequality is from the fact that each vertex of $X$ is contained in at most $K$ of $S_1,\dots, S_n$.
\end{proof}

\subsection{Approximability}


First we analyze the approximation factor. First we analyze the loss caused by the exponential mechanism.

\begin{lemma}\label{lem:expapprox}
We have
\begin{align}
    \E[r(\bar{v})]\geq (1-2\epsilon) \OPT(U).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \Pr[r(\bar{v}) \leq (1-\epsilon)\OPT(U)]
    &= \frac{\sum_{v\in U_d, r(v)\leq (1-\epsilon) \OPT(U)}\exp(r(v)/c)}{\sum_{v\in U_d}\exp(r(v)/c)}\\
    &\leq \frac{|U_d|\exp((1-\epsilon)\OPT(U)/c)}{\sum_{v\in U_d}\exp(r(v)/c)}\\
    &\leq \frac{|U_d|\exp((1-\epsilon)\OPT(U)/c)}{\exp(\OPT(U)/c)}\\
    &= |U_d|\exp(-\epsilon \cdot \OPT(U)/c)\\
    &= |U_d|\cdot \frac{\epsilon}{|U|}\\
    &\leq \epsilon,
\end{align}
where the first inequality is from the algorithm and the last equality is from the definition of $c$.
Therefore, we have
\begin{align}
    \E[r(\bar{v})]
    &\geq (1-\epsilon)(1-\epsilon)\OPT(U)\\
    &\geq (1-2\epsilon)\OPT(U).
\end{align}
\end{proof}

We analyze the loss caused by recursion and complete the approximability analysis.

\begin{lemma}\label{lem:approx}
We have
\begin{align}
    \E\left[w(f(U))\right]\geq (1-17\epsilon\log |U|)\OPT(U).
\end{align}
\end{lemma}
\begin{proof}
We prove by induction on $|U|$. If $|U|=1$, the statement is clear.
For $|U|>1$, we have
\begin{align}
    \E\left[w(f(U))\right]
    &= \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left(\E\left[w(f(U_{-v}))\right]+w(v)+\E\left[w(f(U_{+v}))\right]\right)\right]\\
    &\geq \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left((1-17\epsilon \log |U_{-v}|)\OPT(U_{-v})+w(v)+(1-17\epsilon \log |U_{+v}|)\OPT(U_{+v})\right)\right]\\
    &\geq \left(1-17\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]\left(\OPT(U_{-v})+w(v)+\OPT(U_{+v})\right)\right]\\
    &\geq \left(1-17\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[\sum_{v\in U_d}\Pr[v=\bar{v}]r(v)\right]\\
    &= \left(1-17\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right) \E\left[r(\bar{v})\right]\\
    &\geq \left(1-17\epsilon \log \left(\frac{3}{4}\OPT(U)\right)\right)(1-2\epsilon)\OPT(U)\\
    &\geq \left(1-17\epsilon\log \left(\frac{3}{4}\OPT(U)\right)-2\epsilon \right)\OPT(U)\\
    &\geq (1-17\epsilon\log \OPT(U))\OPT(U),
\end{align}
where the first inequality is from the induction hypothesis, the third inequality is from the definition of $r(v)$, the fourth inequality is from Lemma~\ref{lem:expapprox}, and the last inequality is from $17\log\left(\frac{4}{3}\right)\geq 2$.
\end{proof}

\subsection{Average Sensitivity}

Next we analyze the sensitivity. We denote $r(v)$ in the Algorithm~\ref{alg:main} on the instance $U\setminus S_i$ by $r^i(v)$.

To evaluate the earth mover's distance, we recursively transport probability mass. We transport probability mass so that the case of same choices of $c$, $d$, and $\bar{v}$ correspond to each other. For these cases, We recursively transport probability mass from $\mathcal{A}(f(U_{-v}))$ to $\mathcal{A}(f(U^i_{-v}))$ and from $\mathcal{A}(f(U_{+v}))$ to $\mathcal{A}(f(U^i_{+v}))$. The remaining probability mass is transported arbitrarily.

First, we analyze the impact to the average sensitivity of sampling parameters $c$ and $d$ in the algorithm. The following lemma is useful.

\begin{lemma}\label{lem:benri}
Let $t>0$ be a real number and $p$ (resp. $p^i$) be a parameter in an algorithm for the instance $U$ (resp. $U^i$), sampled from the uniform distribution on $[B,(1+t)B]$ (resp. $[B^i,(1+t)B^i]$). Then, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq \frac{1}{tB}\int_{B}^{(1+t)B}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^i=\hat{p}}(U^i)\right)\right)\mathrm{d}\hat{p}+\frac{1+t}{t}\cdot  \sum_{i=1}^{n}\left|1-\frac{B^i}{B}\right|.
\end{align}
\end{lemma}
\begin{proof}
For $i=1,\dots, n$, we have
\begin{align}
    &\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq \int_{[B,(1+t)B]\cap [B^i,(1+t)B^i]}\left(\min\left(\frac{1}{tB},\frac{1}{tB^i}\right)\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^i=\hat{p}}(U^i)\right) + \max\left(0,\frac{1}{tB}-\frac{1}{tB^i}\right)n\right)\mathrm{d}\hat{p}\\
    &\quad \quad + \int_{[B,(1+t)B]\setminus [B^i,(1+t)B^i]}\frac{1}{tB}n\mathrm{d}\hat{p}\\
    &\leq \int_{B}^{(1+t)B}\frac{1}{tB}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^i=\hat{p}}(U^i)\right)n\mathrm{d}\hat{p}\label{eq:uniform1}\\
    &\quad \quad + \int_{B}^{(1+t)B}\max\left(0,\frac{1}{tB}-\frac{1}{tB^i}\right)n\mathrm{d}\hat{p} + \int_{[B,(1+t)B]\setminus [B^i,(1+t)B^i]}\frac{1}{tB}n\mathrm{d}\hat{p}, \label{eq:uniform2}
\end{align}
where the first inequality is a probability transportation that the case $p=\hat{p}$ is corresponded to the case $p^i=\hat{p}$.
Now, if $B^i\leq B$, we have
\begin{align}
    (\ref{eq:uniform2})
    &= 0 + \int_{(1+t)B^i}^{(1+t)B}\frac{1}{tB}n\mathrm{d}\hat{p}\\
    &=\frac{(1+t)(B-B^i)}{tB}|U|=\frac{1+t}{t}\cdot \left|1-\frac{B^i}{B}\right|n.
\end{align}
Otherwise, we have
\begin{align}
    (\ref{eq:uniform2})
    &= \int_{B}^{(1+t)B}\left(\frac{1}{tB}-\frac{1}{tB^i}\right)n\mathrm{d}\hat{p} + \int_{B}^{B^i}\frac{1}{tB}n\mathrm{d}\hat{p}\\
    &=\left(\left(\frac{1}{tB}-\frac{1}{tB^i}\right)tB+\frac{B^i-B}{tB}\right)n\\
    &=\left(\frac{1}{B^i}+\frac{1}{tB}\right)(B^i-B)n\leq \frac{1+t}{t}\cdot \left|1-\frac{B^i}{B}\right|n.
\end{align}
Therefore, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq \frac{1}{n}\sum_{i=1}^{n}\int_{B}^{(1+t)B}\left(\frac{1}{tB}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^i=\hat{p}}(U^i)\right)\right)\mathrm{d}\hat{p}+\frac{1}{n}\sum_{i=1}^{n}\frac{1+t}{t}\cdot \left|1-\frac{B^i}{B}\right|n\\
    &= \frac{1}{tB}\int_{B}^{(1+t)B}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{p=\hat{p}}(U),\mathcal{A}|_{p^i=\hat{p}}(U^i)\right)\right)\mathrm{d}\hat{p}+\frac{1+t}{t}\cdot  \sum_{i=1}^{n}\left|1-\frac{B^i}{B}\right|.
\end{align}
\end{proof}


%First, let us fix the values of $c=c^i=\hat{c}$ and $d=d^i=\hat{d}$. Let $\mathcal{A}_{\hat{c},\hat{d}}(U)$ be the output distribution of Algorithm~\ref{alg:main} when $c=\hat{c}$ and $d=\hat{d}$ are sampled.
%For simplicity, we simply write $\Pr[\bar{v}=v|c=\hat{c},d=\hat{d}]$ (resp. $\Pr[\bar{v}^i=v|c^i=\hat{c},d^i=\hat{d}]$) by $\Pr[\bar{v}=v]$ (resp. $\Pr[\bar{v}^i=v]$).


%Now let us evaluate the impact to sample $c$ and $d$.
%First, we bound the impact to the average sensitivity of choosing parameters from uniform distribution.

We evaluate the impact of sampling $c$.

\begin{lemma}
We have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq\sup_{\hat{c}\in [B,2B]}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^i=\hat{c}}(U^i)\right)\right)+8K\log\left(|U|\epsilon^{-1}\right),
\end{align}
where $B=\frac{\epsilon\OPT(U)}{\log\left(|U|\epsilon^{-1}\right)}$.
\end{lemma}
\begin{proof}
For $i=1,\dots, n$, let $B^i=\frac{\epsilon\OPT(U^i)}{\log(|U^i|\epsilon^{-1})}$. Then, by applying Lemma~\ref{lem:benri}, we obtain
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq \frac{1}{2B}\int_{B}^{2B}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^i=\hat{c}}(U^i)\right)\right)\mathrm{d}\hat{c}+2\cdot \sum_{i=1}^{n}\left|1-\frac{B^i}{B}\right|\\
    &\leq\sup_{\hat{c}\in [B,2B]}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^i=\hat{c}}(U^i)\right)\right)+2\cdot \sum_{i=1}^{n}\frac{1}{B}\left|B-B^i\right|.\label{eq:cerror1}
\end{align}
Now, we have
\begin{align}
    \frac{1}{B}\left|B-B^i\right|
    &=\frac{1}{B}\left|\frac{\epsilon\OPT(U^i)}{\log(|U^i|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log\left(|U|\epsilon^{-1}\right)}\right|\\
    &\leq \frac{1}{B}\left|\frac{\epsilon\OPT(U^i)}{\log(|U^i|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U^i|\epsilon^{-1})}\right|
    +\frac{1}{B}\left|\frac{\epsilon\OPT(U)}{\log(|U^i|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log\left(|U|\epsilon^{-1}\right)}\right|,\label{eq:cerror2}
\end{align}
where the inequality is from triangular inequality.
Now, we have
\begin{align}
    \sum_{i=1}^{n}\frac{1}{B}\left|\frac{\epsilon\OPT(U^i)}{\log(|U^i|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log(|U^i|\epsilon^{-1})}\right|
    &= \sum_{i=1}^{n}\frac{\log\left(|U|\epsilon^{-1}\right)}{\log((|U|-|S_i|)\epsilon^{-1})}\left(1-\frac{\OPT(U^i)}{\OPT(U)}\right)\\
    &\leq \max\left(\frac{K|U|}{|U|-1},K\right)\cdot \left(\frac{\log\left(|U|\epsilon^{-1}\right)}{\log(\epsilon^{-1})}\cdot 1\right)\\
    &\leq 2K\log\left(|U|\epsilon^{-1}\right),\label{eq:cerror3}
\end{align}
\ynote{I can't follow from (45) to (46).}
where the second inequality is from convexity of $\frac{1}{\log((|U|-x)\epsilon^{-1})}$ over $x$, $\sum_{i=1}^{n}(|U|-|S_i|)\leq K|U|$, and $|U|-|S_i|\geq 1$, and the third inequality is from $|U|\geq 2$ and $\epsilon < 0.2$.
Furthermore, we have
\begin{align}
    \sum_{i=1}^{n}\frac{1}{B}\left|\frac{\epsilon\OPT(U)}{\log(|U^i|\epsilon^{-1})}-\frac{\epsilon\OPT(U)}{\log\left(|U|\epsilon^{-1}\right)}\right|
    &= \sum_{i=1}^{n}\log\left(|U|\epsilon^{-1}\right)\left(\frac{1}{\log((|U|-|S_i|)\epsilon^{-1})}-\frac{1}{\log\left(|U|\epsilon^{-1}\right)}\right)\\
    &\leq \log\left(|U|\epsilon^{-1}\right)\cdot\left(\frac{K|U|}{|U|-1}\cdot \left(\frac{1}{\log(\epsilon^{-1})}-\frac{1}{\log\left(|U|\epsilon^{-1}\right)}\right)\right)\\
    &\leq 2K\log\left(|U|\epsilon^{-1}\right),\label{eq:cerror4}
\end{align}
where the first inequality is from convexity of $\frac{1}{\log((|U|-x)\epsilon^{-1})}$ over $x$, $\sum_{i=1}^{n}(|U|-|S_i|)\leq K|U|$, and $|U|-|S_i|\geq 1$, and the second inequality is from $|U|\geq 2$ and $\epsilon < 0.2$. Combining (\ref{eq:cerror1}), (\ref{eq:cerror2}), (\ref{eq:cerror3}), and (\ref{eq:cerror4}) proves the lemma.
\end{proof}


We evaluate the impact of sampling $d$.
\begin{lemma}\label{lem:impact_cd}
We have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq\sup_{\hat{c}\in [B,2B]}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c}, d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)\right)\mathrm{d}\hat{d}\right)+9K\log\left(|U|\epsilon^{-1}\right),
\end{align}
where $B=\frac{\epsilon\OPT(U)}{\log\left(|U|\epsilon^{-1}\right)}$.
\end{lemma}
\begin{proof}
We have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^i=\hat{c}}(U^i))\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c},d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)\right)\mathrm{d}\hat{d}+3\cdot \sum_{i=1}^{n}\left|1-\frac{\frac{1}{2}(|U|-|S_i|)}{\frac{1}{2}|U|}\right|\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c},d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)\right)\mathrm{d}\hat{d}+3K,
\end{align}
where the first inequality is from Lemma~\ref{lem:benri}, and the second inequality is from Lemma~\ref{lem:hoge} \ynote{put in}.
Therefore, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq\sup_{\hat{c}\in [B,2B]}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c}}(U),\mathcal{A}|_{c^i=\hat{c}}(U^i)\right)\right)+8K\log\left(|U|\epsilon^{-1}\right)\\
    &\leq\sup_{\hat{c}\in [B,2B]}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c},d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)\right)\mathrm{d}\hat{d}+3K\right)+8K\log\left(|U|\epsilon^{-1}\right)\\
    &\leq\sup_{\hat{c}\in [B,2B]}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c},d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)\right)\mathrm{d}\hat{d}\right)+9K\log\left(|U|\epsilon^{-1}\right).
\end{align}
\end{proof}

Now, we concentrate on evaluating the value
\begin{align}
    \frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c},d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)
\end{align}
for fixed $\hat{c}$ and $\hat{d}$. From now on, if it is clear from the context, we omit the symbols that represents the conditioning of these parameter; we simply denote $\mathcal{A}|_{c=\hat{c},d=\hat{d}}(U)$ (resp. $\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)$) by $\mathcal{A}(U)$ (resp. $\mathcal{A}(U^i)$) and $\Pr[\bar{v}=v|c=\hat{c}, d=\hat{d}]$ (resp. $\Pr[\bar{v}=v^i|c^i=\hat{c}, d^i=\hat{d}]$) by $\Pr[\bar{v}=v]$ (resp. $\Pr[\bar{v}=v^i]$).

Now, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}(U),\mathcal{A}(U^i)\right)\\
    &\leq \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\cdot n\\
    &\quad \quad + \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U\setminus S_i}\min\left(\Pr[\bar{v}=v],\Pr[\bar{v}^i=v]\right)\left(\EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)+\EM\left(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v})\right)\right)\\
    &\leq \sum_{i=1}^{n}\sum_{v\in S_i}\Pr[\bar{v}=v] + \sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\label{eq:sumprob}\\
    &\quad \quad + \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\Pr[\bar{v}=v]\left(\EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)+\EM\left(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v})\right)\right)\label{eq:sumprob2}.
\end{align}
Since $\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)$ is positive only if $v\in U_d$, in the last inequality we can take the summation over $v\in U_d\setminus S_i$ instead of $v\in U\setminus S_i$.


Let us evaluate the terms of (\ref{eq:sumprob}). The first term is simple.
\begin{lemma}\label{lem:deletev}
For any choice of $c$ and $d$, we have
\begin{align}
    \sum_{i=1}^{n}\sum_{v\in S_i}\Pr[\bar{v}=v]\leq K.
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \sum_{i=1}^{n}\sum_{v\in S_i}\Pr[\bar{v}=v]=\sum_{i=1}^{n}\Pr[\bar{v}\in S_i]\leq K,
\end{align}
where the inequality is from the assumption that each element of $U$ is contained in at most $K$ of $S_1,\dots, S_n$.
\end{proof}

Let us evaluate the second term. Now, for $v\in U_d\setminus S_i$, we have
\begin{align}
    &\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\\
    &= \max\left(0,\frac{\exp(r(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}^i}\exp(r^i(v')/c)}\right)\\
    &\leq \frac{\exp(r(v)/c)-\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}+\max\left(0,\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}^i}\exp(r^i(v')/c)}\right)\label{eq:pseudotriangle},
\end{align}
where the equality is from the algorithm and the inequality is from the inequality
\begin{align}
    \max(0,b-a)\leq (b-x)+\max(0,x-a)
\end{align}
that holds for $x\leq b$.

Let us give some intuition for these terms. Consider removing $S_i$. The first term of (\ref{eq:pseudotriangle}) represents the decrease of the value $\Pr[\bar{v}=v]$ caused by $r(v)>r^i(v)$, which happens when $S_i$ crosses all maximum chains that contains $v$. The second term of (\ref{eq:pseudotriangle}) represents the decrease of the value $\Pr[\bar{v}=v]$ caused by the increase of the denominator $\sum_{v\in U_{d}}\exp(r(v)/c)$ of the exponential mechanism, which happens if $U_{d}\subsetneq U_{d}^i$ holds.




The next lemma evaluates the impact of the first term of (\ref{eq:pseudotriangle}).
\begin{lemma}\label{lem:triangle_1}
For $c=c^i$ and $d=d^i$, we have
\begin{align}
    \sum_{i=1}^{n}\sum_{v\in U_{d}\setminus S_i}\frac{\exp(r(v)/c)-\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}\leq K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right).
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \frac{\exp(r(v)/c)-\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}
    &= \Pr[\bar{v}=v]\left(1-\frac{\exp(r^i(v)/c)}{\exp(r(v)/c)}\right)\\
    &= \Pr[\bar{v}=v]\left(1-\exp\left(\frac{-(r(v)-r^i(v))}{c}\right)\right)\\
    &\leq \Pr[\bar{v}=v]\cdot \frac{r(v)-r^i(v)}{c},\label{eq:exptolinear}
\end{align}
where the first equality is from the algorithm and the inequality is from $1-\exp(-x)\leq x$.
Therefore, we have
\begin{align}
    \sum_{i=1}^{n}\sum_{v\in U_{d}\setminus S_i}\frac{\exp(r(v)/c)-\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}
    &\leq \sum_{v\in U_{d}}\Pr[\bar{v}=v]\sum_{i\colon S_i\not \ni v} \frac{r(v)-r^i(v)}{c}\\
    &\leq \sum_{v\in U_{d}}\Pr[\bar{v}=v]\cdot \frac{Kr(v)}{c}\\
    &\leq \frac{K}{c} \cdot \OPT(U)\\
    &\leq K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right),
\end{align}
where the first inequality is from (\ref{eq:exptolinear}), the second inequality is from Lemma~\ref{??} \ynote{put in}, the third inequality is from $r(v)\leq \OPT(U)$ and the last inequality is from the definition of $c$.
\end{proof}

The next lemma evaluates the impact of the second term of (\ref{eq:pseudotriangle}).
\begin{lemma}\label{lem:triangle_2}
For $c=c^i$ \ynote{what does this mean?}, we have
\begin{align}
    &\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\max\left(0,\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}^i}\exp(r^i(v')/c)}\right)\right)\mathrm{d}d
    \leq 4K.
\end{align}
\end{lemma}
\begin{proof}
First, we have
\begin{align}
    &\max\left(0,\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}^i}\exp(r^i(v')/c)}\right)\\
    &\leq \max\left(0,\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d+|S_i|}}\exp(r^i(v')/c)}\right)\\
    &\leq \max\left(0,\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d+|S_i|}}\exp(r(v')/c)}\right)\\
    &= \frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d+|S_i|}}\exp(r(v')/c)}\\
    &\leq \frac{\exp(r(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r(v)/c)}{\sum_{v'\in U_{d+|S_i|}}\exp(r(v')/c)},\label{eq:errord1}
\end{align}
where the first inequality is from $U^i_{d}\subseteq U_{d+|S_i|}$ that is from $\max\left(|U^i_{-v}|,|U^i_{+v}|\right)\geq \max\left(|U_{-v}|,|U_{+v}|\right)+|S_i|$, the second and the last inequality is from $r^i(v)\leq r(v)$, and the equality is from $U_d\subseteq U_{d+|S_i|}$.

By taking the expectation over $d$, we have
\begin{align}
    &\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\max\left(0,\frac{\exp(r(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}^i}\exp(r(v')/c)}\right)\right)\mathrm{d}d\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\left(\frac{\exp(r(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r(v)/c)}{\sum_{v'\in U_{d+|S_i|}}\exp(r(v')/c)}\right)\right)\mathrm{d}d\\
    &=\sum_{i=1}^{n}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+|S_i|}\sum_{v\in U_d\setminus S_i}\frac{\exp(r(v)/c)}{\sum_{v'\in U_d}\exp(r(v')/c)}\mathrm{d}d-\int_{\frac{3}{4}|U|}^{\frac{3}{4}|U|+|S_i|}\sum_{v\in U_d\setminus S_i}\frac{\exp(r(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}\mathrm{d}d\right)\\
    &\leq \sum_{i=1}^{n}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{1}{2}|U|+|S_i|}\sum_{v\in U_d\setminus S_i}\frac{\exp(r(v)/c)}{\sum_{v'\in U_d}\exp(r(v')/c)}\mathrm{d}d\right)\\
    &\leq \sum_{i=1}^{n}\frac{4}{|U|}\cdot |S_i| \leq \frac{4}{|U|}\cdot K|U|=4K,
\end{align}
\ynote{I can't follow the derivations from (87) to (88) and from (89) to (90).}
where the first inequality is from (\ref{eq:errord1}) and the fourth inequality is from Lemma~\ref{??} \ynote{put in}.
\end{proof}


Combining (\ref{eq:pseudotriangle}), Lemma~\ref{lem:triangle_1} and Lemma~\ref{lem:triangle_2} yields the following.
\begin{lemma}\label{lem:deteletriangle}
For $c=c^i$, we have
\begin{align}
    \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\right)\mathrm{d}d\leq 2K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right).
\end{align}
\end{lemma}
\begin{proof}
By applying Lemma~\ref{lem:triangle_1} and Lemma~\ref{lem:triangle_2} on (\ref{eq:pseudotriangle}), we have
\begin{align}
    &\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\right)\mathrm{d}d\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\left(\frac{\exp(r(v)/c)-\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}\right.\right.\\
    &\quad \quad \left.\left.+\max\left(0,\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}}\exp(r(v')/c)}-\frac{\exp(r^i(v)/c)}{\sum_{v'\in U_{d}^i}\exp(r^i(v')/c)}\right)\right)\right)\mathrm{d}d\\
    &\leq \frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right)\mathrm{d}d+4K\\
    &= K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right)+4K\leq 2K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right),
\end{align}
where the first inequality is from (\ref{eq:pseudotriangle}), the second inequality is from Lemma~\ref{lem:triangle_1} and Lemma~\ref{lem:triangle_2}, and the last inequality is from $\epsilon<0.2$.
\end{proof}

\begin{comment}
Now we have the following lemma.
\begin{lemma}
We have
\begin{align}
    \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right))\leq hoge.
\end{align}
\end{lemma}
\begin{proof}
Let $B=\frac{\epsilon \OPT(U)}{\log\left(|U|\epsilon^{-1}\right)}$. Then, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\\
    &\leq \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U}\sup_{\hat{c}\in [B,2B]}\left(\max\left(0,\Pr[\bar{v}=v|c=\hat{c}]-\Pr[\bar{v}^i=v|c^i=\hat{c}]\right)\right)+\frac{M}{n}\cdot \left(8K\log\left(|U|\epsilon^{-1}\right)\right)\\
    &\leq \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U}\sup_{\hat{c}\in [B,2B]}\left(\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\frac{4}{|U|}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right))\mathrm{d}\hat{d}\right)+\frac{M}{n}\cdot \left(8K\log\left(|U|\epsilon^{-1}\right)\right)\\
    &\leq
\end{align}
\end{proof}
\end{comment}


We prove the following holds by induction on $|U|$.
\begin{align}
    \frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}(U),\mathcal{A}(U^i)\right)\leq 25\epsilon^{-1}\log^2\left(|U|\epsilon^{-1}\right).\label{eq:ind_hyp}
\end{align}

Now we evaluate the last term.
\begin{lemma}\label{lem:recurse}
Let $k$ be an integer and assume (\ref{eq:ind_hyp}) holds for $|U|<k$. Then, for $|U|=k$, $c=c^i$ and $d=d^i$, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U_{d}\setminus S_i}\Pr[\bar{v}=v]\left(\EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)+\EM(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v}))\right)\leq 25\epsilon^{-1}\log^2\left(\frac{3}{4}|U|\epsilon^{-1}\right).
\end{align}
\end{lemma}
\begin{proof}
Let $i\in \{1,\dots, n\}$ and $v\in U_{d}\setminus S_i$. Since $S_i$ is an antichain, at least one of $S_i\cap U_{-v}$ and $S_i\cap U_{+v}$ is empty. If $S_i\cap U_{-v}=\emptyset$, we have $U_{-v}=U^i_{-v}$ and therefore
\begin{align}
    \EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)=0.
\end{align}
If $S_i\cap U_{+v}=\emptyset$, we have $U_{+v}=U^i_{+v}$ and therefore
\begin{align}
    \EM\left(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v})\right)=0.
\end{align}

Therefore, from induction hypothesis, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U_{d}\setminus S_i}\Pr[\bar{v}=v]\left(\EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)+\EM\left(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v})\right)\right)\\
    &=\frac{1}{n}\sum_{v\in U_{d}}\Pr[\bar{v}=v]\left(\sum_{i\colon S_i\cap U_{-v}\neq \emptyset}\EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)+\sum_{i\colon S_i\cap U_{+v}\neq \emptyset}\EM\left(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v})\right)\right)\\
    &\leq \frac{1}{n}\sum_{v\in U_{d}}\Pr[\bar{v}=v]\left(\left(\left|\{i| S_i\cap U_{-v}\neq \emptyset\}\right|+\left|\{i| S_i\cap U_{-v}\neq \emptyset\}\right|\right)\cdot 25\epsilon^{-1}\log^2\left(\frac{3}{4}|U|\epsilon^{-1}\right)\right)\\
    &\leq \frac{1}{n}\left(n\cdot 25\epsilon^{-1}\log^2\left(\frac{3}{4}|U|\epsilon^{-1}\right)\right)= 25\epsilon^{-1}\log^2\left(\frac{3}{4}|U|\epsilon^{-1}\right).
\end{align}
\end{proof}

Now we complete the analysis by combining all above lemmas.

\begin{lemma}\label{lem:combineall}
We have
\begin{align}
    \frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\leq 25K\epsilon^{-1}\log^2\left(|U|\epsilon^{-1}\right).
\end{align}
\end{lemma}
\begin{proof}
If $|U|=1$, the statement is clear. For $|U|\geq 2$, we have
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM(\mathcal{A}(U),\mathcal{A}(U^i))\\
    &\leq \sup_{\hat{c}\in [B,2B]}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}|_{c=\hat{c}, d=\hat{d}}(U),\mathcal{A}|_{c^i=\hat{c},d^i=\hat{d}}(U^i)\right)\right)\mathrm{d}\hat{d}\right)+9K\log\left(|U|\epsilon^{-1}\right)\\
    &\leq \sup_{\hat{c}\in [B,2B]}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(\sum_{i=1}^{n}\sum_{v\in S_i}\Pr[\bar{v}=v]+ \sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^i=v]\right)\right.\right.\\
    &\quad \quad \left.\left.+ \frac{1}{n}\sum_{i=1}^{n}\sum_{v\in U_d\setminus S_i}\Pr[\bar{v}=v]\left(\EM\left(\mathcal{A}(U_{-v}),\mathcal{A}(U^i_{-v})\right)+\EM\left(\mathcal{A}(U_{+v}),\mathcal{A}(U^i_{+v})\right)\right)\right)\mathrm{d}\hat{d}\right)+9K\log\left(|U|\epsilon^{-1}\right)\\
    &\leq \sup_{\hat{c}\in [B,2B]}\left(\frac{4}{|U|}\int_{\frac{1}{2}|U|}^{\frac{3}{4}|U|}\left(K + 25K\epsilon^{-1}\log\left(\frac{3}{4}|U|\epsilon^{-1}\right)\log n\right)\mathrm{d}\hat{d}+2K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right)\right)+9K\log\left(|U|\epsilon^{-1}\right)\\
    &= K+25K\epsilon^{-1}\log^2\left(\frac{3}{4}|U|\epsilon^{-1}\right)+2K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right)+9K\log\left(|U|\epsilon^{-1}\right)\\
    &\leq \left(25\log\left(\frac{3}{4}|U|\epsilon^{-1}\right)+3\right)K\epsilon^{-1}\log\left(|U|\epsilon^{-1}\right)\\
    &\leq 25K\epsilon^{-1}\log^2\left(|U|\epsilon^{-1}\right),
\end{align}
where the first inequality is Lemma~\ref{lem:impact_cd}, the second inequality is from (\ref{eq:sumprob2}), the third inequality is from Lemma~\ref{lem:deletev}, Lemma~\ref{lem:deteletriangle} and Lemma~\ref{lem:recurse}, the fourth inequality is from $\epsilon<0.2$ and the last inequality is from $25\log\left(\frac{4}{3}\right)\geq 3$. Therefore the induction is completed and the lemma is proved.
\end{proof}

Now we obtain our main result.

\begin{theorem}\label{thm:main}
There is an algorithm to maximum weight chain problem on DAG with approximation ratio $1-\delta$ and average sensitivity $O(K\delta^{-1}\log^3 |V|)$.
\end{theorem}
\begin{proof}
If $\delta^{-1}>|V|$, the theorem clearly holds because the average sensitivity is at most $|V|\leq O(K\delta^{-1}\log^3 |V|)$. Therefore, without loss of generality we can assume $\delta^{-1}\leq |V|$.
Let $B=17\delta^{-1}\log(|V|)$. The algorithm $\mathcal{A}'$ samples a parameter $\epsilon^{-1}$ in algorithm from uniform distribution over $[B,2B]$ and apply the algorithm. Then, from Lemma~\ref{lem:approx}, the approximation ratio is at most $1-\delta$. The average sensitivity is bounded as
\begin{align}
    &\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}'(V),\mathcal{A}'(V^i)\right)\\
    &\leq \frac{1}{B}\int_{B}^{2B}\left(\frac{1}{n}\sum_{i=1}^{n}\EM\left(\mathcal{A}'|_{\epsilon^{-1}=b}(V),\mathcal{A}'|_{\epsilon^{-1}=b}(V^i)\right)\right)\mathrm{d}b
    +2\cdot \sum_{i=1}^{n}\left|1-\frac{\log(|V|-|S_i|)}{\log(|V|)}\right|\\
    &\leq \frac{1}{B}\int_{B}^{2B}\left(25Kb\log^2\left(|V|b\right)\right)\mathrm{d}b
    +2\cdot \sum_{i=1}^{n}\left(1-\frac{\log(|V|-|S_i|)}{\log(|V|)}\right)\\
    &\leq 50KB\log^2\left(2|V|B\right)+2\cdot \sum_{i=1}^{n}\left(1-\frac{\log(|V|-|S_i|)}{\log(|V|)}\right)\\
    &\leq 50KB\log^2\left(2|V|B\right)+2\cdot 1\cdot \frac{K|V|}{|V|-1}\\
    &\leq 50KB\log^2\left(2|V|B\right)+4K\\
    &\leq 54KB\log^2\left(2|V|B\right)\leq O(K\delta^{-1}\log |V|\log^2 \left(|V|\delta^{-1})\right)\leq O(K\delta^{-1}\log^3 |V|),
\end{align}
where the first inequality is from Lemma~\ref{lem:benri}, the second inequality is from Lemma~\ref{lem:combineall}, the fourth inequality is from the convexity of $\log x$, and the last inequality is from $\delta^{-1}\leq |V|$.
\end{proof}


==> old/kukan.tex <==

\begin{algorithm}[t!]
\caption{Less-sensitive Maximum Weight Chain $f(U)$}
\begin{algorithmic}[1]\label{alg:kukan}
\STATE Sample $c$ from the uniform distribution over $\left[\frac{\epsilon \OPT(U)}{\log(|U|\epsilon^{-1})},2\cdot \frac{\epsilon \OPT(U)}{\log(|U|\epsilon^{-1})} \right]$
\STATE Sample $d$ from the uniform distribution over $\left[\frac{1}{2}|U|,\frac{3}{4}|U|\right]$
\IF{$U=\emptyset$}
    \RETURN $\emptyset$
\ENDIF
\FOR{$v\in U$}
    \STATE Let $r(v)$ be the maximum value such that root-$v$ path is ``heavy''
\ENDFOR
\STATE Let $U_d$ be the set of the vertices with $\max\left(|U_{-v}|,|U_{+v}|\right)\leq d$
\STATE Sample $\bar{v}\in U_d$ with probability proportional to $\exp(r(\bar{v})/c)$
\RETURN $f(U_{-\bar{v}})\cup \{\bar{v}\}\cup f(U_{+\bar{v}})$
\end{algorithmic}
\end{algorithm}

Each node of a tree is one of the following types.
\begin{itemize}
    \item Leaf node. This corresponds to an element of the original array.
    \item Merge node. This corresponds to the transition $X\to YZ$.
    \item Match node. This corresponds to the transition $X\to (X)$.
\end{itemize}
The objective value is the number of match nodes.


\begin{lemma}
Approximability.
\end{lemma}
\begin{proof}
Atode. Tabun exp mech surudake.
\end{proof}

Next we analyze the average sensitivity.

\begin{lemma}
We have
\begin{align}
    \sum_{u\in U}\sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^u=v]\right)\leq hoge.
\end{align}
\end{lemma}
\begin{proof}

\end{proof}



==> old/sagyouyou.tex <==
Let $G=(V,E)$ be a transitive directed acyclic graph. For a vertex $v\in V$, let $(-\infty, v)$ be the set of vertices from which there is an edge to $v$, and $(v,\infty)$ be the set of vertices to which there is an edge from $v$. For two vertices $u,v\in V$, let $(u,v)=(u,\infty)\cap (-\infty,v)$. For simplicity, we write $V=(-\infty, \infty)$.

\begin{algorithm}[t!]
\caption{Less-sensitive Maximum Weight Chain $f(U)$}
\begin{algorithmic}[1]\label{alg:main}
\STATE Sample $c$ from the uniform distribution over $\left[\frac{\log(|U|\epsilon^{-1})}{\epsilon \OPT(U)},2\frac{\log(|U|\epsilon^{-1})}{\epsilon \OPT(U)} \right]$
\IF{$U=\emptyset$}
    \RETURN $\emptyset$
\ENDIF
\FOR{$v\in U$}
    \STATE Let $a=\OPT(U_{-v})$, $b=\OPT(U_{+v})$
    \IF{$a+b+1$ is odd}
        \STATE $r(v)\leftarrow \frac{2}{3}(a+b+\min(a,b))+1$
    \ELSE
        \STATE $r(v)\leftarrow \frac{2}{3}(a+b+\min(a,b))+\frac{4}{3}$
    \ENDIF
\ENDFOR
\STATE Sample $\bar{v}$ with probability proportional to $\exp(cr(\bar{v}))$
\RETURN $f(U_{-v})\cup \{v\}\cup f(U_{+v})$
\end{algorithmic}
\end{algorithm}

The answer is $f(V)$.

\begin{lemma}
We have $\max_{v\in U} r(v) = \OPT(U)$.
\end{lemma}
\begin{proof}
Let $C=(v_1,\dots, v_{\OPT(U)})$ be the chain that attains $\OPT(U)$. Let $v=v_{\lceil \frac{\OPT(U)}{2}\rceil}$. Then, if $\OPT(U)$ is odd, we have
\begin{align}
    r(v)&=\frac{2}{3}\left(\OPT(U)+\frac{\OPT(U)-3}{2}\right)+1=\OPT(U),
\end{align}
and if $\OPT(U)$ is even, we have
\begin{align}
    r(v)&=\frac{2}{3}\left(\OPT(U)+\frac{\OPT(U)-4}{2}\right)+\frac{4}{3}=\OPT(U).
\end{align}
Therefore $\max_{v\in U} r(v) \geq \OPT(U)$ holds.

Conversely, let $v$ be a vertex, $a=\OPT(U_{-v})$ and $b=\OPT(U_{+v})$. Then, if $a+b+1$ is odd, we have
\begin{align}
    r(v)&=\frac{2}{3}(a+b+\min(a,b))+1\leq \frac{2}{3}\left(\OPT(U)-1+\frac{\OPT(U)-1}{2}\right)+1 = \OPT(U),
\end{align}
and if $a+b+1$ is even, we have
\begin{align}
    r(v)&=\frac{2}{3}(a+b+\min(a,b))+\frac{4}{3}\leq \frac{2}{3}\left(\OPT(U)-1+\frac{\OPT(U)-2}{2}\right)+\frac{4}{3} = \OPT(U).
\end{align}
Therefore $\max_{v\in U} r(v) \leq \OPT(U)$ holds and the lemma is proved.
\end{proof}

First we analyze the approximation factor. First we analyze the loss by the exponential mechanism.

\begin{lemma}
We have 
\begin{align}
    \E[r(\bar{v})]\geq (1-2\epsilon) \OPT(U).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    \Pr[r(\bar{v}) \leq (1-\epsilon)\OPT(U)]
    &=\frac{\sum_{v\in U, r(v)\leq (1-\epsilon \OPT(U))}\exp(cr(v))}{\sum_{v\in U}\exp(cr(v))}\\
    &\leq \frac{|U|\exp((1-\epsilon)c\cdot \OPT(U))}{\sum_{v\in U}\exp(cr(v))}\\
    &\leq \frac{|U|\exp((1-\epsilon)c\cdot \OPT(U))}{\exp(c\cdot \OPT(U))}\\
    &= |U|\exp(-\epsilon c\cdot \OPT(U))\\
    &\leq \epsilon.
\end{align}

Therefore, we have
\begin{align}
    \E[r(\bar{v})]
    &\geq (1-\epsilon)(1-\epsilon)\OPT(U)\\
    &\geq (1-2\epsilon)\OPT(U).
\end{align}
\end{proof}


\begin{lemma}
We have 
\begin{align}
    \E[r(\bar{v})]\geq (1-2\epsilon) \OPT(U).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
    \Pr[r(\bar{v}) \leq (1-\epsilon)\OPT(U)]
    &=\frac{\sum_{v\in U, r(v)\leq (1-\epsilon \OPT(U))}\exp(cr(v))}{\sum_{v\in U}\exp(cr(v))}\\
    &\leq \frac{|U|\exp((1-\epsilon)c\cdot \OPT(U))}{\sum_{v\in U}\exp(cr(v))}\\
    &\leq \frac{|U|\exp((1-\epsilon)c\cdot \OPT(U))}{\exp(c\cdot \OPT(U))}\\
    &= |U|\exp(-\epsilon c\cdot \OPT(U))\\
    &\leq \epsilon.
\end{align}

Therefore, we have
\begin{align}
    \E[r(\bar{v})]
    &\geq (1-\epsilon)(1-\epsilon)\OPT(U)\\
    &\geq (1-2\epsilon)\OPT(U).
\end{align}
\end{proof}

Next, we analyze the loss by the recursion.

\begin{lemma}
We have
\begin{align}
    \E\left[|f(U)|\right]\geq (1-8\epsilon\log \OPT(U))\OPT(U).
\end{align}
\end{lemma}
\begin{proof}
We prove by induction on $\OPT(U)$. If $\OPT(U)=0$, the statement is clear.
We have
\begin{align}
    \Pr\left[\OPT(U_{-\bar{v}})\geq \frac{2}{3}\OPT(U)\right]
    &= \frac{\sum_{v\in U, \OPT(U_{-\bar{v}})\geq \frac{2}{3}\OPT(U)}\exp(cr(v))}{\sum_{v\in U}\exp(cr(v))}\\
    &\leq \frac{|U|\exp\left(c\cdot \frac{8}{9}\OPT(U)\right)}{\sum_{v\in U}\exp(cr(v))}\\
    &\leq \frac{|U|\exp\left(c\cdot \frac{8}{9}\OPT(U)\right)}{\exp(c\cdot \OPT(U))}\\
    &= |U|\exp\left(-c\cdot \frac{1}{9}\OPT(U)\right)\\
    &\leq |U|\exp\left(-\epsilon c\cdot \OPT(U)\right)\\
    &\leq \epsilon.
\end{align}


Now, we have
\begin{align}
    \E\left[|f(U)|\right]
    &= \E\left[\sum_{v\in U}\Pr[v=\bar{v}]\left(\E\left[|f(U_{-v})|\right]+\E\left[|f(U_{+v})|\right]\right)\right]+1\\
    &\geq \E\left[\sum_{v\in U}\Pr[v=\bar{v}]\left(\E\left[|f(U_{-v})|\right]+\E\left[|f(U_{+v})|\right]\right)\right]+1\\
    &\geq \E\left[\sum_{v\in U, |U_{-v}|, |U_{+v}|\leq \frac{2}{3}\OPT(U)}\Pr[v=\bar{v}]\left(\E\left[|f(U_{-v})|\right]+\E\left[|f(U_{+v})|\right]\right)\right]+1\\
    &\geq \left(1-8\epsilon\log \left(\frac{2}{3}\OPT(U)\right)\right)\E\left[\sum_{v\in U, |U_{-v}|, |U_{+v}|\leq \frac{2}{3}\OPT(U)}\Pr[v=\bar{v}](\OPT(U_{-v})+\OPT(U_{+v})+1)\right]\\
    &\geq \left(1-8\epsilon\log \left(\frac{2}{3}\OPT(U)\right)\right)\E\left[\sum_{v\in U}\Pr[v=\bar{v}](\OPT(U_{-v})+\OPT(U_{+v})+1)-2\epsilon \OPT(U)\right]\\
    &\geq \left(1-8\epsilon\log \left(\frac{2}{3}\OPT(U)\right)\right)\E\left[s(\bar{v})-2\epsilon \OPT(U)\right]\\
    &\geq \left(1-8\epsilon\log \left(\frac{2}{3}\OPT(U)\right)\right)(1-4\epsilon)\OPT(U)\\\
    &\geq (1-8\epsilon\log \OPT(U))\OPT(U).
\end{align}
\end{proof}


Next we analyze the sensitivity. We denote $r(v)$ in the Algorithm~\ref{alg:main} on the instance $U\setminus \{u\}$ by $r^u(v)$.

To evaluate the earth mover's distance, we recursively transport the probability. We transport the probability so that the case of same choice of the pivots correspond to each other. For these cases, We recursively transport the probability from $\mathcal{A}(f(U_{-v}))$ to $\mathcal{A}(f(U^u_{-v}))$ and from $\mathcal{A}(f(U_{+v}))$ to $\mathcal{A}(f(U^u_{+v}))$.

Now, we have
\begin{align}
    &\EM(\mathcal{A}(f(U)),\mathcal{A}(f(U^u)))\\
    &= \sum_{v\in U\setminus \{u\}}\min\left(\Pr[\bar{v}=v],\Pr[\bar{v}^u=v]\right)\left(\EM(\mathcal{A}(f(U_{-v})),\mathcal{A}(f(U^u_{-v})))+\EM(\mathcal{A}(f(U_{+v})),\mathcal{A}(f(U^u_{+v})))\right)\\
    &+ \sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\OPT(U).
\end{align}

\begin{lemma}
For $u,v\in U$, we have $r^u(v)\geq r(v)-\frac{5}{3}$.
\end{lemma}
\begin{proof}
Let $a=\OPT(U_{-v}), b=\OPT(U_{+v})$ and $a^u=\OPT(U^u_{-v}), b^u=\OPT(U^u_{+v})$. Now, we have
\begin{align}
    r(v)-r^u(v)
    &\leq \frac{2}{3}\left(\left(a+b+\min(a,b)\right)-\left(a^u+b^u+\min(a^u,b^u)\right)\right)+\left(\frac{4}{3}-1\right)\\
    &\leq \frac{4}{3}+\frac{1}{3}=\frac{5}{3}.
\end{align}
\end{proof}

\begin{lemma}
We have
\begin{align}
    \sum_{v\in U}\max\left(0,\Pr[\bar{v}=v]-\Pr[\bar{v}^{u}=v]\right)\leq hoge.
\end{align}
\end{lemma}
\begin{proof}
For $v\in U$ with $v\neq u$, we have
\begin{align}
    \frac{\Pr[\bar{v}^u=v]}{\Pr[\bar{v}=v]}
    &=\frac{\frac{\exp(cr^u(v))}{\sum_{v'\in U^u}\exp(cr^u(v'))}}{\frac{\exp(cr(v))}{\sum_{v'\in U}\exp(cr(v'))}}\\
    &\geq \frac{\exp(cr^u(v))}{\exp(cr(v))}\\
    &= \exp\left(-c(r(v)-r^u(v))\right)\\
    &\geq \exp\left(-\frac{5}{3}c\right)\\
    &\geq 1-\frac{5}{3}c\\
    &\geq 1-\frac{10\log(|U|\epsilon^{-1})}{3\epsilon \OPT(U)}.
\end{align}
\end{proof}
